Relevance meets Diversity: A User-Centric Framework for Knowledge Exploration through Recommendations

Providing recommendations that are both relevant and diverse is a key consideration of modern recommender systems. Optimizing both of these measures presents a fundamental trade-off, as higher diversity typically comes at the cost of relevance, resulting in lower user engagement. Existing recommendation algorithms try to resolve this trade-off by combining the two measures, relevance and diversity, into one aim and then seeking recommendations that optimize the combined objective, for a given number of items to recommend. Traditional approaches, however, do not consider the user interaction with the recommended items. In this paper, we put the user at the central stage, and build on the interplay between relevance, diversity, and user behavior. In contrast to applications where the goal is solely to maximize engagement, we focus on scenarios aiming at maximizing the total amount of knowledge encountered by the user. We use diversity as a surrogate of the amount of knowledge obtained by the user while interacting with the system, and we seek to maximize diversity. We propose a probabilistic user-behavior model in which users keep interacting with the recommender system as long as they receive relevant recommendations, but they may stop if the relevance of the recommended items drops. Thus, for a recommender system to achieve a high-diversity measure, it will need to produce recommendations that are both relevant and diverse. Finally, we propose a novel recommendation strategy that combines relevance and diversity by a copula function. We conduct an extensive evaluation of the proposed methodology over multiple datasets, and we show that our strategy outperforms several state-of-the-art competitors. Our implementation is publicly available at https://github.com/EricaCoppolillo/EXPLORE.

==> KuaiRec-2.0_small/deterministic_jaccard_users_scores_table.tex <==
\resizebox{\textwidth}{!}{\begin{tabular}{c c c c c c c c c}
$k$ & $B$ & Strategy & \multicolumn{1}{c}{$D(C)$} & \multicolumn{1}{c}{$\textit{cov(C)}$} & \multicolumn{1}{c}{\textit{steps}} &\multicolumn{1}{c}{$\Delta_{\mathbbm{E[\textit{D}]}}$} & \multicolumn{1}{c}{$\Delta_{\mathbbm{E[\textit{cov}]}}$} &\multicolumn{1}{c}{$\Delta_{\mathbbm{E[\textit{steps}}]}$} \\ 
\midrule
\multirow{21}{*}{2} & \multirow{7}{*}{10} & \multirow{1}{*}{Relevance} & 0.52 & 0.09 & 3.55 & 0.81 &0.77 &0.03 \\ 
\cmidrule{3-9}
& &\multirow{1}{*}{Interacted distance} & \textbf{1.44} & 0.1 & 3.2 & \textbf{0.49} &0.75 &0.13 \\ 
& &\multirow{1}{*}{Coverage} & 0.8 & \textbf{0.32} & 3.29 & 0.71 &\textbf{0.2} &0.1 \\ 
\cmidrule{3-9}
& &\multirow{1}{*}{MMR} & 1.06 & 0.1 & 3.13 & 0.62 &0.75 &0.14 \\ 
& &\multirow{1}{*}{DUM} & 0.53 & 0.09 & 3.56 & 0.81 &0.77 &0.03 \\ 
& &\multirow{1}{*}{DPP} & 0.88 & 0.09 & 3.55 & 0.69 &0.77 &0.03 \\ 
& &\multirow{1}{*}{DGREC} & 1.11 & 0.14 & 2.86 & 0.6 &0.65 &0.22 \\ 
\cmidrule{2-9}
& \multirow{7}{*}{20} & \multirow{1}{*}{Relevance} & 0.78 & 0.11 & 5.13 & 0.81 &0.79 &0.03 \\ 
\cmidrule{3-9}
& &\multirow{1}{*}{Interacted distance} & \textbf{2.07} & 0.13 & 4.52 & \textbf{0.5} &0.75 &0.15 \\ 
& &\multirow{1}{*}{Coverage} & 1.2 & \textbf{0.41} & 4.66 & 0.71 &\textbf{0.2} &0.12 \\ 
\cmidrule{3-9}
& &\multirow{1}{*}{MMR} & 1.59 & 0.14 & 4.43 & 0.61 &0.73 &0.16 \\ 
& &\multirow{1}{*}{DUM} & 0.78 & 0.12 & 5.12 & 0.81 &0.77 &0.03 \\ 
& &\multirow{1}{*}{DPP} & 1.3 & 0.12 & 5.12 & 0.68 &0.77 &0.03 \\ 
& &\multirow{1}{*}{DGREC} & 1.59 & 0.18 & 4.13 & 0.61 &0.65 &0.22 \\ 
\cmidrule{2-9}
& \multirow{7}{*}{40} & \multirow{1}{*}{Relevance} & 1.15 & 0.15 & 7.33 & 0.81 &0.77 &0.04 \\ 
\cmidrule{3-9}
& &\multirow{1}{*}{Interacted distance} & \textbf{2.95} & 0.16 & 6.43 & \textbf{0.5} &0.75 &0.15 \\ 
& &\multirow{1}{*}{Coverage} & 1.76 & \textbf{0.52} & 6.57 & 0.7 &\textbf{0.19} &0.14 \\ 
\cmidrule{3-9}
& &\multirow{1}{*}{MMR} & 2.28 & 0.18 & 6.23 & 0.62 &0.72 &0.18 \\ 
& &\multirow{1}{*}{DUM} & 1.15 & 0.16 & 7.35 & 0.81 &0.75 &0.03 \\ 
& &\multirow{1}{*}{DPP} & 1.87 & 0.15 & 7.36 & 0.69 &0.77 &0.03 \\ 
& &\multirow{1}{*}{DGREC} & 2.23 & 0.24 & 6.01 & 0.63 &0.63 &0.21 \\ 
\midrule
\multirow{21}{*}{10} & \multirow{7}{*}{10} & \multirow{1}{*}{Relevance} & 0.55 & 0.1 & 3.55 & 0.8 &0.75 &0.03 \\ 
\cmidrule{3-9}
& &\multirow{1}{*}{Interacted distance} & \textbf{1.27} & 0.1 & 2.89 & \textbf{0.55} &0.75 &0.21 \\ 
& &\multirow{1}{*}{Coverage} & 0.81 & \textbf{0.28} & 3.19 & 0.71 &\textbf{0.3} &0.13 \\ 
\cmidrule{3-9}
& &\multirow{1}{*}{MMR} & 0.92 & 0.1 & 3.05 & 0.67 &0.75 &0.17 \\ 
& &\multirow{1}{*}{DUM} & 0.6 & 0.13 & \textbf{3.58} & 0.79 &0.67 &\textbf{0.02} \\ 
& &\multirow{1}{*}{DPP} & 1.02 & 0.08 & 3.54 & 0.64 &0.8 &0.03 \\ 
& &\multirow{1}{*}{DGREC} & 0.62 & 0.1 & 2.25 & 0.78 &0.75 &0.39 \\ 
\cmidrule{2-9}
& \multirow{7}{*}{20} & \multirow{1}{*}{Relevance} & 0.82 & 0.13 & 5.1 & 0.8 &0.75 &0.04 \\ 
\cmidrule{3-9}
& &\multirow{1}{*}{Interacted distance} & \textbf{1.75} & 0.12 & 3.94 & \textbf{0.58} &0.77 &0.26 \\ 
& &\multirow{1}{*}{Coverage} & 1.19 & \textbf{0.37} & 4.48 & 0.71 &\textbf{0.28} &0.15 \\ 
\cmidrule{3-9}
& &\multirow{1}{*}{MMR} & 1.38 & 0.13 & 4.22 & 0.66 &0.75 &0.2 \\ 
& &\multirow{1}{*}{DUM} & 0.89 & 0.18 & 5.13 & 0.78 &0.65 &0.03 \\ 
& &\multirow{1}{*}{DPP} & 1.5 & 0.1 & 5.1 & 0.64 &0.81 &0.04 \\ 
& &\multirow{1}{*}{DGREC} & 0.95 & 0.13 & 3.16 & 0.77 &0.75 &0.4 \\ 
\cmidrule{2-9}
& \multirow{7}{*}{40} & \multirow{1}{*}{Relevance} & 1.21 & 0.18 & 7.35 & 0.8 &0.72 &0.03 \\ 
\cmidrule{3-9}
& &\multirow{1}{*}{Interacted distance} & \textbf{2.44} & 0.15 & 5.47 & \textbf{0.59} &0.77 &0.28 \\ 
& &\multirow{1}{*}{Coverage} & 1.73 & \textbf{0.46} & 6.31 & 0.71 &\textbf{0.28} &0.17 \\ 
\cmidrule{3-9}
& &\multirow{1}{*}{MMR} & 1.98 & 0.17 & 5.83 & 0.67 &0.74 &0.23 \\ 
& &\multirow{1}{*}{DUM} & 1.32 & 0.23 & 7.33 & 0.78 &0.64 &0.04 \\ 
& &\multirow{1}{*}{DPP} & 2.15 & 0.13 & 7.3 & 0.64 &0.8 &0.04 \\ 
& &\multirow{1}{*}{DGREC} & 1.39 & 0.17 & 4.47 & 0.77 &0.74 &0.41 \\ 
\midrule
\multirow{21}{*}{20} & \multirow{7}{*}{10} & \multirow{1}{*}{Relevance} & 0.61 & 0.11 & 3.57 & 0.78 &0.72 &0.02 \\ 
\cmidrule{3-9}
& &\multirow{1}{*}{Interacted distance} & \textbf{1.25} & 0.1 & 2.89 & \textbf{0.55} &0.75 &0.21 \\ 
& &\multirow{1}{*}{Coverage} & 0.82 & \textbf{0.27} & 3.19 & 0.71 &\textbf{0.32} &0.13 \\ 
\cmidrule{3-9}
& &\multirow{1}{*}{MMR} & 0.92 & 0.1 & 3.07 & 0.67 &0.75 &0.16 \\ 
& &\multirow{1}{*}{DUM} & 0.79 & 0.15 & 3.57 & 0.72 &0.62 &0.02 \\ 
& &\multirow{1}{*}{DPP} & 1.02 & 0.08 & 3.55 & 0.64 &0.8 &0.03 \\ 
& &\multirow{1}{*}{DGREC} & 0.61 & 0.1 & 2.28 & 0.78 &0.75 &0.38 \\ 
\cmidrule{2-9}
& \multirow{7}{*}{20} & \multirow{1}{*}{Relevance} & 0.91 & 0.15 & 5.13 & 0.78 &0.71 &0.03 \\ 
\cmidrule{3-9}
& &\multirow{1}{*}{Interacted distance} & \textbf{1.75} & 0.13 & 3.97 & \textbf{0.58} &0.75 &0.25 \\ 
& &\multirow{1}{*}{Coverage} & 1.21 & \textbf{0.35} & 4.49 & 0.71 &\textbf{0.32} &0.15 \\ 
\cmidrule{3-9}
& &\multirow{1}{*}{MMR} & 1.38 & 0.13 & 4.25 & 0.66 &0.75 &0.2 \\ 
& &\multirow{1}{*}{DUM} & 1.18 & 0.2 & 5.16 & 0.71 &0.61 &0.03 \\ 
& &\multirow{1}{*}{DPP} & 1.5 & 0.1 & 5.1 & 0.64 &0.81 &0.04 \\ 
& &\multirow{1}{*}{DGREC} & 0.91 & 0.13 & 3.12 & 0.78 &0.75 &0.41 \\ 
\cmidrule{2-9}
& \multirow{7}{*}{40} & \multirow{1}{*}{Relevance} & 1.34 & 0.19 & 7.34 & 0.77 &0.7 &0.04 \\ 
\cmidrule{3-9}
& &\multirow{1}{*}{Interacted distance} & \textbf{2.43} & 0.16 & 5.52 & \textbf{0.59} &0.75 &0.27 \\ 
& &\multirow{1}{*}{Coverage} & 1.75 & \textbf{0.44} & 6.3 & 0.71 &\textbf{0.32} &0.17 \\ 
\cmidrule{3-9}
& &\multirow{1}{*}{MMR} & 1.98 & 0.17 & 5.89 & 0.67 &0.74 &0.23 \\ 
& &\multirow{1}{*}{DUM} & 1.69 & 0.26 & 7.33 & 0.72 &0.6 &0.04 \\ 
& &\multirow{1}{*}{DPP} & 2.16 & 0.13 & 7.33 & 0.64 &0.8 &0.04 \\ 
& &\multirow{1}{*}{DGREC} & 1.32 & 0.16 & 4.41 & 0.78 &0.75 &0.42 \\ 
\midrule
\end{tabular}}
\caption{Results on KuaiRec-2.0. The best scores with a statistical significance $p<0.05$ are highlighted in bold.}
\label{tab:jaccard_users_KuaiRec-2.0_small_scores_table}
 

==> KuaiRec-2.0_small/partial_scores_table.tex <==
\begin{table*}
 \centering 
\resizebox{0.6\textwidth}{!}{\begin{tabular}{c|c|c|c|c|c|c|c|c}
\hline 
% Dataset & Patience & Rec Strategy & \multicolumn{1}{c|}{R(C)} & \multicolumn{1}{c|}{cov(C)} & \multicolumn{1}{c|}{steps} &\multicolumn{1}{c|}{$\delta_R$} & \multicolumn{1}{c|}{$\delta_{cov}$} &\multicolumn{1}{c}{$\delta_{steps}$} \\ 
% \hline
\hline
\multirow{21}{*}{\rotatebox{90}{KuaiRec-2.0}} & \multirow{7}{*}{10} & \multirow{1}{*}{relevance} & 0.55 & 0.1 & \underline{3.55} & 0.8 &0.75 &\underline{0.03} \\ 
\cline{3-9}
& &\multirow{1}{*}{interacted distance w relevance} & \textbf{1.27} & 0.1 & 2.89 & \textbf{0.55} &0.75 &0.21 \\ 
& &\multirow{1}{*}{coverage w relevance} & 0.81 & \textbf{0.28} & 3.19 & 0.71 &\textbf{0.3} &0.13 \\ 
\cline{3-9}
& &\multirow{1}{*}{mmr} & 0.92 & 0.1 & 3.05 & 0.67 &0.75 &0.17 \\ 
& &\multirow{1}{*}{dpp} & \underline{1.02} & 0.08 & 3.54 & \underline{0.64} &0.8 &\underline{0.03} \\ 
& &\multirow{1}{*}{dum} & 0.6 & \underline{0.13} & \textbf{3.58} & 0.79 &\underline{0.67} &\textbf{0.02} \\ 
& &\multirow{1}{*}{dgrec} & 0.62 & 0.1 & 2.25 & 0.78 &0.75 &0.39 \\ 
\hhline{~========}
& \multirow{7}{*}{20} & \multirow{1}{*}{relevance} & 0.82 & 0.13 & \underline{5.1} & 0.8 &0.75 &\underline{0.04} \\ 
\cline{3-9}
& &\multirow{1}{*}{interacted distance w relevance} & \textbf{1.75} & 0.12 & 3.94 & \textbf{0.58} &0.77 &0.26 \\ 
& &\multirow{1}{*}{coverage w relevance} & 1.19 & \textbf{0.37} & 4.48 & 0.71 &\textbf{0.28} &0.15 \\ 
\cline{3-9}
& &\multirow{1}{*}{mmr} & 1.38 & 0.13 & 4.22 & 0.66 &0.75 &0.2 \\ 
& &\multirow{1}{*}{dpp} & \underline{1.5} & 0.1 & \underline{5.1} & \underline{0.64} &0.81 &\underline{0.04} \\ 
& &\multirow{1}{*}{dum} & 0.89 & \underline{0.18} & \textbf{5.13} & 0.78 &\underline{0.65} &\textbf{0.03} \\ 
& &\multirow{1}{*}{dgrec} & 0.95 & 0.13 & 3.16 & 0.77 &0.75 &0.4 \\ 
\hhline{~========}
& \multirow{7}{*}{40} & \multirow{1}{*}{relevance} & 1.21 & 0.18 & \textbf{7.35} & 0.8 &0.72 &\textbf{0.03} \\ 
\cline{3-9}
& &\multirow{1}{*}{interacted distance w relevance} & \textbf{2.44} & 0.15 & 5.47 & \textbf{0.59} &0.77 &0.28 \\ 
& &\multirow{1}{*}{coverage w relevance} & 1.73 & \textbf{0.46} & 6.31 & 0.71 &\textbf{0.28} &0.17 \\ 
\cline{3-9}
& &\multirow{1}{*}{mmr} & 1.98 & 0.17 & 5.83 & 0.67 &0.74 &0.23 \\ 
& &\multirow{1}{*}{dpp} & \underline{2.15} & 0.13 & 7.3 & \underline{0.64} &0.8 &\underline{0.04} \\ 
& &\multirow{1}{*}{dum} & 1.32 & \underline{0.23} & \underline{7.33} & 0.78 &\underline{0.64} &\underline{0.04} \\ 
& &\multirow{1}{*}{dgrec} & 1.39 & 0.17 & 4.47 & 0.77 &0.74 &0.41 \\ 
\hline
\end{tabular}}
\caption{Experiments over KuaiRec-2.0 adopting jaccard distance in terms of users. Results have been obtained by averaging 20 independent trails. Bold and underline values represent the best and second-best scores, respectively.}
\label{tab:jaccard_users_KuaiRec-2.0_small_scores_table}
\end{table*}

==> ablation_table.tex <==
\begin{table}
 \centering 
\resizebox{\columnwidth}{!}{\begin{tabular}{c c c c c c}
{} & Strategy & Relevance & \multicolumn{1}{c}{$D(C)$} & \multicolumn{1}{c}{$cov(C)$} & \multicolumn{1}{c}{$\textit{steps}$} \\ 
 \cmidrule{1-6} 
\multirow{8}{*}{\rotatebox{90}{Movielens-1M}} & \multirow{4}{*}{Interacted distance} & w& 5.24 & 0.38 & 5.29 \\ 
& & w/o& 3.57 & 0.33 & 3.69 \\ 
\cmidrule(lr){4-6}
& & $\Delta$ & \textbf{+1.67} & \textbf{+0.05} & \textbf{+1.6} \\ 
& & $\Delta_w$ & \textbf{+0.32} & \textbf{+0.13} & \textbf{+0.3} \\ 
\cmidrule(lr){3-6}
& \multirow{4}{*}{Coverage} & w& 4.78 & 0.76 & 5.04 \\ 
& & w/o& 3.87 & 0.74 & 4.11 \\ 
\cmidrule(lr){4-6}
& & $\Delta$ & \textbf{+0.91} & \textbf{+0.02} & \textbf{+0.93} \\ 
& & $\Delta_w$ & \textbf{+0.19} & \textbf{+0.03} & \textbf{+0.18} \\ 
\cmidrule(lr){1-6}
\multirow{8}{*}{\rotatebox{90}{Coat}} & \multirow{4}{*}{Interacted distance} & w& 3.84 & 0.37 & 4.55 \\ 
& & w/o& 3.17 & 0.33 & 3.69 \\ 
\cmidrule(lr){4-6}
& & $\Delta$ & \textbf{+0.67} & \textbf{+0.04} & \textbf{+0.86} \\ 
& & $\Delta_w$ & \textbf{+0.17} & \textbf{+0.11} & \textbf{+0.19} \\ 
\cmidrule(lr){3-6}
& \multirow{4}{*}{Coverage} & w& 3.72 & 0.38 & 4.53 \\ 
& & w/o& 3.03 & 0.33 & 3.63 \\ 
\cmidrule(lr){4-6}
& & $\Delta$ & \textbf{+0.69} & \textbf{+0.05} & \textbf{+0.9} \\ 
& & $\Delta_w$ & \textbf{+0.19} & \textbf{+0.13} & \textbf{+0.2} \\ 
\cmidrule(lr){1-6}
\multirow{8}{*}{\rotatebox{90}{KuaiRec-2.0}} & \multirow{4}{*}{Interacted distance} & w& 1.75 & 0.12 & 3.94 \\ 
& & w/o& 1.3 & 0.08 & 2.52 \\ 
\cmidrule(lr){4-6}
& & $\Delta$ & \textbf{+0.45} & \textbf{+0.04} & \textbf{+1.42} \\ 
& & $\Delta_w$ & \textbf{+0.26} & \textbf{+0.33} & \textbf{+0.36} \\ 
\cmidrule(lr){3-6}
& \multirow{4}{*}{Coverage} & w& 1.19 & 0.37 & 4.48 \\ 
& & w/o& 1.16 & 0.34 & 3.59 \\ 
\cmidrule(lr){4-6}
& & $\Delta$ & \textbf{+0.03} & \textbf{+0.03} & \textbf{+0.89} \\ 
& & $\Delta_w$ & \textbf{+0.03} & \textbf{+0.08} & \textbf{+0.2} \\ 
\cmidrule{1-6}
\end{tabular}}
\caption{Results obtained with $k = 10$ and $B = 20$, by including (\rm w\textbf{) and excluding (}\rm w/o\textbf{) relevance from our strategies. We report the absolute ($\Delta$) and relative change ($\Delta_w$) by fixing the score with relevance as the reference. Positive variations have been highlighted in bold.}}
\label{tab:ablation_table}
\end{table}

==> coat/ali_alphas_table.tex <==
\begin{table*}
 \centering 
\resizebox{0.4\textwidth}{!}{\begin{tabular}{c c c c c c c c c c}
\midrule 
k & Patience & Rec Strategy  & $\alpha$ &  \multicolumn{1}{c}{R(C)} & \multicolumn{1}{c}{cov(C)} & \multicolumn{1}{c}{steps} &\multicolumn{1}{c}{$\delta_R$} & \multicolumn{1}{c}{$\delta_{cov}$} &\multicolumn{1}{c}{$\delta_{steps}$} \\ 
\midrule
\multirow{30}{*}{2} & \multirow{10}{*}{10} & \multirow{5}{*}{Interacted distance} & \multirow{1}{*}{-1} & 2.819 & 0.304 & 3.285 & 0.208 &0.098 &0.103 \\ 
& & &\multirow{1}{*}{-0.5} & 2.84 & \underline{0.305} & 3.311 & 0.202 &\underline{0.095} &\underline{0.095} \\ 
& & &\multirow{1}{*}{0} & \textbf{2.848} & \textbf{0.306} & \textbf{3.325} & \textbf{0.2} &\textbf{0.092} &\textbf{0.092} \\ 
& & &\multirow{1}{*}{0.5} & 2.83 & 0.304 & 3.309 & 0.205 &0.098 &0.096 \\ 
& & &\multirow{1}{*}{1} & \underline{2.845} & \underline{0.305} & \underline{3.323} & \underline{0.201} &\underline{0.095} &\textbf{0.092} \\ 
\cmidrule{3-10}
& &\multirow{5}{*}{Coverage} & \multirow{1}{*}{-1} & \underline{2.756} & \underline{0.312} & \underline{3.341} & \underline{0.226} &\underline{0.074} &\underline{0.087} \\ 
& & &\multirow{1}{*}{-0.5} & \textbf{2.767} & \textbf{0.313} & \textbf{3.348} & \textbf{0.223} &\textbf{0.071} &\textbf{0.085} \\ 
& & &\multirow{1}{*}{0} & 2.736 & 0.311 & 3.326 & 0.232 &0.077 &0.091 \\ 
& & &\multirow{1}{*}{0.5} & 2.714 & 0.309 & 3.3 & 0.238 &0.083 &0.098 \\ 
& & &\multirow{1}{*}{1} & 2.704 & 0.307 & 3.289 & 0.24 &0.089 &0.101 \\ 
\cmidrule{2-10}
& \multirow{10}{*}{20} & \multirow{5}{*}{Interacted distance} & \multirow{1}{*}{-1} & \underline{4.046} & \textbf{0.383} & 4.682 & \underline{0.228} &\textbf{0.127} &0.116 \\ 
& & &\multirow{1}{*}{-0.5} & 4.044 & \underline{0.382} & 4.684 & 0.229 &\underline{0.13} &0.115 \\ 
& & &\multirow{1}{*}{0} & 4.043 & 0.381 & \underline{4.698} & 0.229 &0.132 &\underline{0.113} \\ 
& & &\multirow{1}{*}{0.5} & 4.022 & 0.379 & 4.674 & 0.233 &0.137 &0.117 \\ 
& & &\multirow{1}{*}{1} & \textbf{4.066} & \underline{0.382} & \textbf{4.73} & \textbf{0.225} &\underline{0.13} &\textbf{0.106} \\ 
\cmidrule{3-10}
& &\multirow{5}{*}{Coverage} & \multirow{1}{*}{-1} & \textbf{3.861} & \textbf{0.402} & \textbf{4.733} & \textbf{0.264} &\textbf{0.084} &\textbf{0.106} \\ 
& & &\multirow{1}{*}{-0.5} & 3.802 & 0.397 & 4.663 & 0.275 &0.096 &0.119 \\ 
& & &\multirow{1}{*}{0} & \underline{3.849} & \underline{0.401} & \underline{4.724} & \underline{0.266} &\underline{0.086} &\underline{0.108} \\ 
& & &\multirow{1}{*}{0.5} & 3.843 & 0.4 & 4.708 & 0.267 &0.089 &0.111 \\ 
& & &\multirow{1}{*}{1} & 3.722 & 0.387 & 4.589 & 0.29 &0.118 &0.133 \\ 
\cmidrule{2-10}
& \multirow{10}{*}{40} & \multirow{5}{*}{Interacted distance} & \multirow{1}{*}{-1} & 5.63 & \underline{0.473} & 6.565 & 0.258 &\underline{0.176} &0.137 \\ 
& & &\multirow{1}{*}{-0.5} & 5.659 & \underline{0.473} & 6.601 & 0.254 &\underline{0.176} &0.132 \\ 
& & &\multirow{1}{*}{0} & \underline{5.675} & 0.471 & \underline{6.636} & \underline{0.252} &0.179 &\underline{0.128} \\ 
& & &\multirow{1}{*}{0.5} & \textbf{5.728} & \textbf{0.474} & \textbf{6.698} & \textbf{0.245} &\textbf{0.174} &\textbf{0.12} \\ 
& & &\multirow{1}{*}{1} & 5.657 & 0.469 & 6.62 & 0.254 &0.182 &0.13 \\ 
\cmidrule{3-10}
& &\multirow{5}{*}{Coverage} & \multirow{1}{*}{-1} & 5.307 & \textbf{0.512} & 6.602 & \underline{0.3} &\textbf{0.108} &\underline{0.132} \\ 
& & &\multirow{1}{*}{-0.5} & 5.285 & 0.51 & 6.575 & 0.303 &0.111 &0.136 \\ 
& & &\multirow{1}{*}{0} & \underline{5.308} & \underline{0.511} & \underline{6.605} & \underline{0.3} &\underline{0.109} &\underline{0.132} \\ 
& & &\multirow{1}{*}{0.5} & \textbf{5.326} & \textbf{0.512} & \textbf{6.624} & \textbf{0.298} &\textbf{0.108} &\textbf{0.129} \\ 
& & &\multirow{1}{*}{1} & 5.028 & 0.482 & 6.335 & 0.337 &0.16 &0.167 \\ 
\midrule
\multirow{30}{*}{10} & \multirow{10}{*}{10} & \multirow{5}{*}{Interacted distance} & \multirow{1}{*}{-1} & 2.668 & \textbf{0.294} & 3.207 & \underline{0.251} &\textbf{0.128} &0.124 \\ 
& & &\multirow{1}{*}{-0.5} & \textbf{2.675} & \textbf{0.294} & \underline{3.221} & \textbf{0.249} &\textbf{0.128} &\underline{0.12} \\ 
& & &\multirow{1}{*}{0} & 2.649 & 0.292 & 3.191 & 0.256 &0.133 &0.128 \\ 
& & &\multirow{1}{*}{0.5} & \underline{2.672} & \underline{0.293} & \textbf{3.225} & \textbf{0.249} &\underline{0.131} &\textbf{0.119} \\ 
& & &\multirow{1}{*}{1} & 2.617 & 0.289 & 3.183 & 0.265 &0.142 &0.13 \\ 
\cmidrule{3-10}
& &\multirow{5}{*}{Coverage} & \multirow{1}{*}{-1} & \underline{2.593} & \textbf{0.296} & \underline{3.184} & \underline{0.272} &\textbf{0.122} &\underline{0.13} \\ 
& & &\multirow{1}{*}{-0.5} & 2.581 & \underline{0.295} & 3.169 & 0.275 &\underline{0.125} &0.134 \\ 
& & &\multirow{1}{*}{0} & \textbf{2.597} & \textbf{0.296} & \textbf{3.189} & \textbf{0.271} &\textbf{0.122} &\textbf{0.129} \\ 
& & &\multirow{1}{*}{0.5} & 2.588 & \textbf{0.296} & 3.177 & 0.273 &\textbf{0.122} &0.132 \\ 
& & &\multirow{1}{*}{1} & 2.552 & 0.292 & 3.141 & 0.283 &0.133 &0.142 \\ 
\cmidrule{2-10}
& \multirow{10}{*}{20} & \multirow{5}{*}{Interacted distance} & \multirow{1}{*}{-1} & \textbf{3.85} & \textbf{0.368} & \textbf{4.55} & \textbf{0.266} &\textbf{0.162} &\textbf{0.14} \\ 
& & &\multirow{1}{*}{-0.5} & 3.831 & \underline{0.366} & 4.542 & 0.269 &\underline{0.166} &0.142 \\ 
& & &\multirow{1}{*}{0} & 3.831 & \underline{0.366} & 4.534 & 0.269 &\underline{0.166} &0.143 \\ 
& & &\multirow{1}{*}{0.5} & \underline{3.836} & \underline{0.366} & \underline{4.549} & \underline{0.268} &\underline{0.166} &\underline{0.141} \\ 
& & &\multirow{1}{*}{1} & 3.787 & 0.363 & 4.506 & 0.278 &0.173 &0.149 \\ 
\cmidrule{3-10}
& &\multirow{5}{*}{Coverage} & \multirow{1}{*}{-1} & 3.664 & \underline{0.378} & 4.452 & \underline{0.301} &\underline{0.139} &\underline{0.159} \\ 
& & &\multirow{1}{*}{-0.5} & \underline{3.667} & \underline{0.378} & \underline{4.453} & \underline{0.301} &\underline{0.139} &\underline{0.159} \\ 
& & &\multirow{1}{*}{0} & \textbf{3.693} & \textbf{0.38} & \textbf{4.492} & \textbf{0.296} &\textbf{0.134} &\textbf{0.151} \\ 
& & &\multirow{1}{*}{0.5} & 3.637 & 0.376 & 4.426 & 0.306 &0.143 &0.164 \\ 
& & &\multirow{1}{*}{1} & 3.601 & 0.373 & 4.385 & 0.313 &0.15 &0.172 \\ 
\cmidrule{2-10}
& \multirow{10}{*}{40} & \multirow{5}{*}{Interacted distance} & \multirow{1}{*}{-1} & \underline{5.357} & 0.448 & 6.341 & \underline{0.294} &0.219 &0.167 \\ 
& & &\multirow{1}{*}{-0.5} & 5.353 & \underline{0.449} & 6.339 & \underline{0.294} &\underline{0.217} &0.167 \\ 
& & &\multirow{1}{*}{0} & \textbf{5.375} & \textbf{0.45} & \textbf{6.368} & \textbf{0.291} &\textbf{0.216} &\textbf{0.163} \\ 
& & &\multirow{1}{*}{0.5} & \underline{5.357} & 0.447 & \underline{6.358} & \underline{0.294} &0.221 &\underline{0.164} \\ 
& & &\multirow{1}{*}{1} & 5.295 & 0.444 & 6.29 & 0.302 &0.226 &0.173 \\ 
\cmidrule{3-10}
& &\multirow{5}{*}{Coverage} & \multirow{1}{*}{-1} & \underline{5.122} & \textbf{0.483} & 6.259 & \underline{0.325} &\textbf{0.158} &\underline{0.177} \\ 
& & &\multirow{1}{*}{-0.5} & 5.001 & 0.475 & 6.124 & 0.341 &0.172 &0.195 \\ 
& & &\multirow{1}{*}{0} & \textbf{5.125} & \underline{0.482} & \underline{6.266} & \textbf{0.324} &\underline{0.16} &\underline{0.177} \\ 
& & &\multirow{1}{*}{0.5} & 5.12 & 0.481 & \textbf{6.271} & \underline{0.325} &0.162 &\textbf{0.176} \\ 
& & &\multirow{1}{*}{1} & 4.829 & 0.461 & 5.91 & 0.363 &0.196 &0.223 \\ 
\midrule
\multirow{30}{*}{20} & \multirow{10}{*}{10} & \multirow{5}{*}{Interacted distance} & \multirow{1}{*}{-1} & \underline{2.66} & \underline{0.292} & \underline{3.243} & \underline{0.253} &\underline{0.133} &\underline{0.114} \\ 
& & &\multirow{1}{*}{-0.5} & 2.649 & 0.291 & 3.236 & 0.256 &0.136 &0.116 \\ 
& & &\multirow{1}{*}{0} & \textbf{2.673} & \textbf{0.293} & \textbf{3.262} & \textbf{0.249} &\textbf{0.131} &\textbf{0.109} \\ 
& & &\multirow{1}{*}{0.5} & 2.642 & 0.291 & 3.232 & 0.258 &0.136 &0.117 \\ 
& & &\multirow{1}{*}{1} & 2.601 & 0.288 & 3.21 & 0.269 &0.145 &0.123 \\ 
\cmidrule{3-10}
& &\multirow{5}{*}{Coverage} & \multirow{1}{*}{-1} & 2.516 & 0.289 & 3.142 & 0.293 &0.142 &0.142 \\ 
& & &\multirow{1}{*}{-0.5} & 2.498 & 0.287 & 3.133 & 0.298 &0.148 &0.144 \\ 
& & &\multirow{1}{*}{0} & \underline{2.558} & \underline{0.292} & \underline{3.193} & \underline{0.282} &\underline{0.133} &\underline{0.128} \\ 
& & &\multirow{1}{*}{0.5} & \textbf{2.598} & \textbf{0.295} & \textbf{3.242} & \textbf{0.27} &\textbf{0.125} &\textbf{0.114} \\ 
& & &\multirow{1}{*}{1} & 2.502 & 0.287 & 3.122 & 0.297 &0.148 &0.147 \\ 
\cmidrule{2-10}
& \multirow{10}{*}{20} & \multirow{5}{*}{Interacted distance} & \multirow{1}{*}{-1} & 3.773 & \underline{0.362} & 4.529 & 0.28 &\underline{0.175} &0.144 \\ 
& & &\multirow{1}{*}{-0.5} & 3.778 & 0.361 & 4.539 & 0.28 &0.178 &0.143 \\ 
& & &\multirow{1}{*}{0} & \underline{3.78} & \underline{0.362} & \underline{4.552} & \underline{0.279} &\underline{0.175} &\underline{0.14} \\ 
& & &\multirow{1}{*}{0.5} & \textbf{3.794} & \textbf{0.363} & \textbf{4.562} & \textbf{0.276} &\textbf{0.173} &\textbf{0.138} \\ 
& & &\multirow{1}{*}{1} & 3.753 & 0.36 & 4.531 & 0.284 &0.18 &0.144 \\ 
\cmidrule{3-10}
& &\multirow{5}{*}{Coverage} & \multirow{1}{*}{-1} & \textbf{3.683} & \textbf{0.377} & \textbf{4.524} & \textbf{0.298} &\textbf{0.141} &\textbf{0.145} \\ 
& & &\multirow{1}{*}{-0.5} & 3.62 & 0.372 & 4.452 & 0.31 &0.152 &0.159 \\ 
& & &\multirow{1}{*}{0} & \underline{3.654} & \underline{0.374} & 4.492 & \underline{0.303} &\underline{0.148} &\underline{0.151} \\ 
& & &\multirow{1}{*}{0.5} & 3.646 & 0.373 & \underline{4.493} & 0.305 &0.15 &\underline{0.151} \\ 
& & &\multirow{1}{*}{1} & 3.551 & 0.366 & 4.383 & 0.323 &0.166 &0.172 \\ 
\cmidrule{2-10}
& \multirow{10}{*}{40} & \multirow{5}{*}{Interacted distance} & \multirow{1}{*}{-1} & 5.302 & 0.443 & 6.373 & 0.301 &0.228 &0.162 \\ 
& & &\multirow{1}{*}{-0.5} & \underline{5.354} & \underline{0.446} & \underline{6.428} & \underline{0.294} &\underline{0.223} &\underline{0.155} \\ 
& & &\multirow{1}{*}{0} & \textbf{5.375} & \textbf{0.448} & \textbf{6.461} & \textbf{0.291} &\textbf{0.219} &\textbf{0.151} \\ 
& & &\multirow{1}{*}{0.5} & 5.319 & 0.445 & 6.393 & 0.299 &0.224 &0.16 \\ 
& & &\multirow{1}{*}{1} & 5.283 & 0.443 & 6.366 & 0.303 &0.228 &0.163 \\ 
\cmidrule{3-10}
& &\multirow{5}{*}{Coverage} & \multirow{1}{*}{-1} & \textbf{5.087} & \textbf{0.474} & \textbf{6.265} & \textbf{0.329} &\textbf{0.174} &\textbf{0.177} \\ 
& & &\multirow{1}{*}{-0.5} & 4.997 & 0.468 & 6.158 & 0.341 &0.184 &0.191 \\ 
& & &\multirow{1}{*}{0} & \underline{5.067} & \underline{0.472} & \underline{6.249} & \underline{0.332} &\underline{0.177} &\underline{0.179} \\ 
& & &\multirow{1}{*}{0.5} & 5.039 & 0.468 & 6.228 & 0.336 &0.184 &0.182 \\ 
& & &\multirow{1}{*}{1} & 4.814 & 0.454 & 5.931 & 0.365 &0.209 &0.221 \\ 

\end{tabular}}
\caption{Experiments over coat adopting jaccard distance in terms of genres. Results have been obtained by averaging 20 independent trails. Bold and underline values represent the best and second-best scores, respectively.}
\label{tab:jaccard_genres_coat_scores_table}
\end{table*}

==> coat/clayton_alphas_table.tex <==
\begin{table*}
 \centering 
\resizebox{0.3\textwidth}{!}{\begin{tabular}{c c c c c c c c c c}
\midrule 
k & Patience & Rec Strategy  & $\alpha$ &  \multicolumn{1}{c}{R(C)} & \multicolumn{1}{c}{cov(C)} & \multicolumn{1}{c}{steps} &\multicolumn{1}{c}{$\delta_R$} & \multicolumn{1}{c}{$\delta_{cov}$} &\multicolumn{1}{c}{$\delta_{steps}$} \\ 
\midrule
\multirow{48}{*}{2} & \multirow{16}{*}{10} & \multirow{8}{*}{Interacted distance} & \multirow{1}{*}{0.0001} & 2.817 & 0.303 & 3.28 & 0.209 &0.101 &0.104 \\ 
& & &\multirow{1}{*}{0.001} & 2.86 & \underline{0.306} & 3.337 & 0.197 &\underline{0.092} &0.088 \\ 
& & &\multirow{1}{*}{0.01} & \underline{2.862} & \underline{0.306} & \underline{3.342} & \underline{0.196} &\underline{0.092} &\underline{0.087} \\ 
& & &\multirow{1}{*}{0.1} & \textbf{2.871} & \textbf{0.307} & \textbf{3.348} & \textbf{0.194} &\textbf{0.089} &\textbf{0.085} \\ 
& & &\multirow{1}{*}{0.5} & 2.843 & 0.305 & 3.317 & 0.201 &0.095 &0.094 \\ 
& & &\multirow{1}{*}{1} & 2.825 & 0.304 & 3.294 & 0.207 &0.098 &0.1 \\ 
& & &\multirow{1}{*}{2} & 2.857 & \underline{0.306} & 3.326 & 0.198 &\underline{0.092} &0.091 \\ 
& & &\multirow{1}{*}{4} & 2.861 & \underline{0.306} & 3.335 & \underline{0.196} &\underline{0.092} &0.089 \\ 
\cmidrule{3-10}
& &\multirow{8}{*}{Coverage} & \multirow{1}{*}{0.0001} & \underline{2.756} & \underline{0.312} & 3.339 & \underline{0.226} &\underline{0.074} &0.088 \\ 
& & &\multirow{1}{*}{0.001} & 2.718 & 0.309 & 3.3 & 0.237 &0.083 &0.098 \\ 
& & &\multirow{1}{*}{0.01} & \textbf{2.782} & \textbf{0.314} & \textbf{3.373} & \textbf{0.219} &\textbf{0.068} &\textbf{0.078} \\ 
& & &\multirow{1}{*}{0.1} & \underline{2.756} & \underline{0.312} & \underline{3.35} & \underline{0.226} &\underline{0.074} &\underline{0.085} \\ 
& & &\multirow{1}{*}{0.5} & 2.739 & 0.311 & 3.324 & 0.231 &0.077 &0.092 \\ 
& & &\multirow{1}{*}{1} & 2.74 & 0.311 & 3.318 & 0.23 &0.077 &0.093 \\ 
& & &\multirow{1}{*}{2} & 2.738 & 0.311 & 3.326 & 0.231 &0.077 &0.091 \\ 
& & &\multirow{1}{*}{4} & 2.75 & 0.311 & 3.332 & 0.228 &0.077 &0.09 \\ 
\cmidrule{2-10}
& \multirow{16}{*}{20} & \multirow{8}{*}{Interacted distance} & \multirow{1}{*}{0.0001} & \textbf{4.083} & \textbf{0.384} & \textbf{4.737} & \textbf{0.221} &\textbf{0.125} &\textbf{0.105} \\ 
& & &\multirow{1}{*}{0.001} & \underline{4.07} & \underline{0.383} & \underline{4.726} & \underline{0.224} &\underline{0.127} &\underline{0.107} \\ 
& & &\multirow{1}{*}{0.01} & 4.053 & 0.382 & 4.708 & 0.227 &0.13 &0.111 \\ 
& & &\multirow{1}{*}{0.1} & 4.017 & 0.38 & 4.66 & 0.234 &0.134 &0.12 \\ 
& & &\multirow{1}{*}{0.5} & 4.059 & 0.382 & 4.716 & 0.226 &0.13 &0.109 \\ 
& & &\multirow{1}{*}{1} & 4.05 & 0.381 & 4.708 & 0.228 &0.132 &0.111 \\ 
& & &\multirow{1}{*}{2} & 4.057 & 0.381 & 4.722 & 0.226 &0.132 &0.108 \\ 
& & &\multirow{1}{*}{4} & 3.998 & 0.376 & 4.664 & 0.238 &0.143 &0.119 \\ 
\cmidrule{3-10}
& &\multirow{8}{*}{Coverage} & \multirow{1}{*}{0.0001} & 3.835 & 0.399 & 4.701 & 0.269 &0.091 &0.112 \\ 
& & &\multirow{1}{*}{0.001} & \textbf{3.863} & \textbf{0.402} & \textbf{4.734} & \textbf{0.263} &\textbf{0.084} &\textbf{0.106} \\ 
& & &\multirow{1}{*}{0.01} & 3.809 & 0.398 & 4.675 & 0.274 &0.093 &0.117 \\ 
& & &\multirow{1}{*}{0.1} & 3.84 & 0.399 & 4.699 & 0.268 &0.091 &0.112 \\ 
& & &\multirow{1}{*}{0.5} & \underline{3.854} & \underline{0.401} & 4.722 & \underline{0.265} &\underline{0.086} &0.108 \\ 
& & &\multirow{1}{*}{1} & 3.853 & \underline{0.401} & \underline{4.725} & \underline{0.265} &\underline{0.086} &\underline{0.107} \\ 
& & &\multirow{1}{*}{2} & 3.849 & 0.4 & 4.721 & 0.266 &0.089 &0.108 \\ 
& & &\multirow{1}{*}{4} & 3.828 & 0.398 & 4.692 & 0.27 &0.093 &0.114 \\ 
\cmidrule{2-10}
& \multirow{16}{*}{40} & \multirow{8}{*}{Interacted distance} & \multirow{1}{*}{0.0001} & 5.689 & \underline{0.472} & 6.65 & 0.25 &\underline{0.177} &0.126 \\ 
& & &\multirow{1}{*}{0.001} & \textbf{5.746} & \textbf{0.475} & \textbf{6.716} & \textbf{0.242} &\textbf{0.172} &\textbf{0.117} \\ 
& & &\multirow{1}{*}{0.01} & 5.678 & \underline{0.472} & 6.637 & 0.251 &\underline{0.177} &0.128 \\ 
& & &\multirow{1}{*}{0.1} & 5.661 & 0.47 & 6.617 & 0.254 &0.181 &0.13 \\ 
& & &\multirow{1}{*}{0.5} & 5.693 & 0.471 & 6.661 & \underline{0.249} &0.179 &0.125 \\ 
& & &\multirow{1}{*}{1} & 5.625 & 0.467 & 6.58 & 0.258 &0.186 &0.135 \\ 
& & &\multirow{1}{*}{2} & \underline{5.696} & 0.469 & \underline{6.669} & \underline{0.249} &0.182 &\underline{0.124} \\ 
& & &\multirow{1}{*}{4} & 5.673 & 0.465 & 6.656 & 0.252 &0.189 &0.125 \\ 
\cmidrule{3-10}
& &\multirow{8}{*}{Coverage} & \multirow{1}{*}{0.0001} & 5.305 & 0.511 & 6.593 & 0.301 &0.109 &0.134 \\ 
& & &\multirow{1}{*}{0.001} & 5.319 & \underline{0.512} & 6.604 & 0.299 &\underline{0.108} &0.132 \\ 
& & &\multirow{1}{*}{0.01} & \textbf{5.357} & \textbf{0.514} & \textbf{6.664} & \textbf{0.294} &\textbf{0.104} &\textbf{0.124} \\ 
& & &\multirow{1}{*}{0.1} & 5.298 & 0.51 & 6.591 & 0.301 &0.111 &0.134 \\ 
& & &\multirow{1}{*}{0.5} & 5.314 & \underline{0.512} & \underline{6.622} & 0.299 &\underline{0.108} &\underline{0.13} \\ 
& & &\multirow{1}{*}{1} & 5.313 & 0.511 & 6.608 & 0.299 &0.109 &0.132 \\ 
& & &\multirow{1}{*}{2} & 5.319 & 0.51 & 6.62 & 0.299 &0.111 &\underline{0.13} \\ 
& & &\multirow{1}{*}{4} & \underline{5.348} & \underline{0.512} & \textbf{6.664} & \underline{0.295} &\underline{0.108} &\textbf{0.124} \\ 
\midrule
\multirow{48}{*}{10} & \multirow{16}{*}{10} & \multirow{8}{*}{Interacted distance} & \multirow{1}{*}{0.0001} & \textbf{2.72} & \textbf{0.297} & \textbf{3.266} & \textbf{0.236} &\textbf{0.119} &\textbf{0.108} \\ 
& & &\multirow{1}{*}{0.001} & 2.672 & \underline{0.294} & 3.212 & 0.249 &\underline{0.128} &0.122 \\ 
& & &\multirow{1}{*}{0.01} & 2.677 & \underline{0.294} & 3.217 & 0.248 &\underline{0.128} &0.121 \\ 
& & &\multirow{1}{*}{0.1} & \underline{2.691} & \underline{0.294} & 3.232 & \underline{0.244} &\underline{0.128} &0.117 \\ 
& & &\multirow{1}{*}{0.5} & 2.655 & 0.292 & 3.206 & 0.254 &0.133 &0.124 \\ 
& & &\multirow{1}{*}{1} & 2.681 & 0.293 & \underline{3.234} & 0.247 &0.131 &\underline{0.116} \\ 
& & &\multirow{1}{*}{2} & 2.643 & 0.29 & 3.211 & 0.258 &0.139 &0.123 \\ 
& & &\multirow{1}{*}{4} & 2.596 & 0.287 & 3.181 & 0.271 &0.148 &0.131 \\ 
\cmidrule{3-10}
& &\multirow{8}{*}{Coverage} & \multirow{1}{*}{0.0001} & 2.594 & \underline{0.296} & 3.176 & 0.271 &\underline{0.122} &0.132 \\ 
& & &\multirow{1}{*}{0.001} & \underline{2.601} & \textbf{0.297} & \underline{3.201} & \underline{0.269} &\textbf{0.119} &\underline{0.125} \\ 
& & &\multirow{1}{*}{0.01} & 2.572 & 0.294 & 3.158 & 0.278 &0.128 &0.137 \\ 
& & &\multirow{1}{*}{0.1} & 2.581 & 0.295 & 3.173 & 0.275 &0.125 &0.133 \\ 
& & &\multirow{1}{*}{0.5} & 2.569 & 0.294 & 3.166 & 0.278 &0.128 &0.135 \\ 
& & &\multirow{1}{*}{1} & 2.586 & 0.295 & 3.176 & 0.274 &0.125 &0.132 \\ 
& & &\multirow{1}{*}{2} & 2.574 & 0.294 & 3.176 & 0.277 &0.128 &0.132 \\ 
& & &\multirow{1}{*}{4} & \textbf{2.61} & \underline{0.296} & \textbf{3.232} & \textbf{0.267} &\underline{0.122} &\textbf{0.117} \\ 
\cmidrule{2-10}
& \multirow{16}{*}{20} & \multirow{8}{*}{Interacted distance} & \multirow{1}{*}{0.0001} & \textbf{3.884} & \textbf{0.369} & \textbf{4.597} & \textbf{0.259} &\textbf{0.159} &\textbf{0.132} \\ 
& & &\multirow{1}{*}{0.001} & 3.8 & 0.364 & 4.502 & 0.275 &0.171 &0.15 \\ 
& & &\multirow{1}{*}{0.01} & 3.812 & 0.365 & 4.519 & 0.273 &0.168 &0.146 \\ 
& & &\multirow{1}{*}{0.1} & \underline{3.823} & \underline{0.366} & \underline{4.535} & \underline{0.271} &\underline{0.166} &\underline{0.143} \\ 
& & &\multirow{1}{*}{0.5} & 3.782 & 0.363 & 4.487 & 0.279 &0.173 &0.152 \\ 
& & &\multirow{1}{*}{1} & 3.752 & 0.361 & 4.462 & 0.284 &0.178 &0.157 \\ 
& & &\multirow{1}{*}{2} & 3.789 & 0.362 & 4.511 & 0.277 &0.175 &0.148 \\ 
& & &\multirow{1}{*}{4} & 3.755 & 0.36 & 4.495 & 0.284 &0.18 &0.151 \\ 
\cmidrule{3-10}
& &\multirow{8}{*}{Coverage} & \multirow{1}{*}{0.0001} & 3.681 & 0.379 & 4.473 & 0.298 &0.137 &0.155 \\ 
& & &\multirow{1}{*}{0.001} & 3.687 & 0.379 & 4.481 & 0.297 &0.137 &0.154 \\ 
& & &\multirow{1}{*}{0.01} & 3.679 & 0.379 & 4.472 & 0.298 &0.137 &0.155 \\ 
& & &\multirow{1}{*}{0.1} & 3.699 & 0.38 & 4.492 & 0.295 &0.134 &0.151 \\ 
& & &\multirow{1}{*}{0.5} & \underline{3.722} & \underline{0.382} & \underline{4.529} & \underline{0.29} &\underline{0.13} &\underline{0.144} \\ 
& & &\multirow{1}{*}{1} & \textbf{3.736} & \textbf{0.383} & \textbf{4.538} & \textbf{0.288} &\textbf{0.127} &\textbf{0.143} \\ 
& & &\multirow{1}{*}{2} & 3.687 & 0.379 & 4.503 & 0.297 &0.137 &0.149 \\ 
& & &\multirow{1}{*}{4} & 3.632 & 0.374 & 4.464 & 0.307 &0.148 &0.157 \\ 
\cmidrule{2-10}
& \multirow{16}{*}{40} & \multirow{8}{*}{Interacted distance} & \multirow{1}{*}{0.0001} & \underline{5.384} & \underline{0.449} & \underline{6.379} & \underline{0.29} &\underline{0.217} &\underline{0.162} \\ 
& & &\multirow{1}{*}{0.001} & 5.33 & 0.447 & 6.32 & 0.297 &0.221 &0.169 \\ 
& & &\multirow{1}{*}{0.01} & 5.363 & \underline{0.449} & 6.356 & 0.293 &\underline{0.217} &0.165 \\ 
& & &\multirow{1}{*}{0.1} & 5.344 & 0.447 & 6.338 & 0.295 &0.221 &0.167 \\ 
& & &\multirow{1}{*}{0.5} & \textbf{5.406} & \textbf{0.451} & \textbf{6.413} & \textbf{0.287} &\textbf{0.214} &\textbf{0.157} \\ 
& & &\multirow{1}{*}{1} & 5.333 & 0.447 & 6.333 & 0.297 &0.221 &0.168 \\ 
& & &\multirow{1}{*}{2} & 5.264 & 0.442 & 6.269 & 0.306 &0.23 &0.176 \\ 
& & &\multirow{1}{*}{4} & 5.286 & 0.443 & 6.306 & 0.303 &0.228 &0.171 \\ 
\cmidrule{3-10}
& &\multirow{8}{*}{Coverage} & \multirow{1}{*}{0.0001} & 5.107 & 0.481 & 6.249 & 0.327 &0.162 &0.179 \\ 
& & &\multirow{1}{*}{0.001} & 5.116 & 0.482 & 6.256 & 0.325 &0.16 &0.178 \\ 
& & &\multirow{1}{*}{0.01} & \underline{5.13} & \underline{0.483} & 6.277 & \underline{0.324} &\underline{0.158} &0.175 \\ 
& & &\multirow{1}{*}{0.1} & \textbf{5.143} & \textbf{0.484} & \underline{6.284} & \textbf{0.322} &\textbf{0.156} &\underline{0.174} \\ 
& & &\multirow{1}{*}{0.5} & 5.09 & 0.479 & 6.238 & 0.329 &0.165 &0.18 \\ 
& & &\multirow{1}{*}{1} & 5.105 & 0.48 & 6.256 & 0.327 &0.163 &0.178 \\ 
& & &\multirow{1}{*}{2} & 5.067 & 0.476 & 6.222 & 0.332 &0.17 &0.182 \\ 
& & &\multirow{1}{*}{4} & 5.129 & 0.477 & \textbf{6.321} & \underline{0.324} &0.169 &\textbf{0.169} \\ 
\midrule
\multirow{48}{*}{20} & \multirow{16}{*}{10} & \multirow{8}{*}{Interacted distance} & \multirow{1}{*}{0.0001} & 2.653 & \underline{0.291} & \textbf{3.249} & \underline{0.255} &\underline{0.136} &\textbf{0.112} \\ 
& & &\multirow{1}{*}{0.001} & \textbf{2.656} & \textbf{0.292} & \underline{3.245} & \textbf{0.254} &\textbf{0.133} &\underline{0.113} \\ 
& & &\multirow{1}{*}{0.01} & 2.643 & \underline{0.291} & 3.229 & 0.258 &\underline{0.136} &0.118 \\ 
& & &\multirow{1}{*}{0.1} & 2.635 & 0.29 & 3.224 & 0.26 &0.139 &0.119 \\ 
& & &\multirow{1}{*}{0.5} & \underline{2.655} & \underline{0.291} & \textbf{3.249} & \textbf{0.254} &\underline{0.136} &\textbf{0.112} \\ 
& & &\multirow{1}{*}{1} & 2.622 & 0.289 & 3.235 & 0.264 &0.142 &0.116 \\ 
& & &\multirow{1}{*}{2} & 2.594 & 0.286 & 3.205 & 0.271 &0.151 &0.124 \\ 
& & &\multirow{1}{*}{4} & 2.558 & 0.284 & 3.19 & 0.282 &0.157 &0.128 \\ 
\cmidrule{3-10}
& &\multirow{8}{*}{Coverage} & \multirow{1}{*}{0.0001} & \underline{2.553} & \underline{0.291} & 3.185 & \underline{0.283} &\underline{0.136} &0.13 \\ 
& & &\multirow{1}{*}{0.001} & 2.525 & 0.289 & 3.157 & 0.291 &0.142 &0.137 \\ 
& & &\multirow{1}{*}{0.01} & 2.538 & 0.29 & 3.171 & 0.287 &0.139 &0.134 \\ 
& & &\multirow{1}{*}{0.1} & 2.533 & 0.29 & 3.173 & 0.289 &0.139 &0.133 \\ 
& & &\multirow{1}{*}{0.5} & 2.51 & 0.288 & 3.144 & 0.295 &0.145 &0.141 \\ 
& & &\multirow{1}{*}{1} & \textbf{2.583} & \textbf{0.293} & \textbf{3.216} & \textbf{0.274} &\textbf{0.131} &\textbf{0.121} \\ 
& & &\multirow{1}{*}{2} & 2.503 & 0.287 & 3.141 & 0.297 &0.148 &0.142 \\ 
& & &\multirow{1}{*}{4} & 2.543 & 0.29 & \underline{3.198} & 0.286 &0.139 &\underline{0.126} \\ 
\cmidrule{2-10}
& \multirow{16}{*}{20} & \multirow{8}{*}{Interacted distance} & \multirow{1}{*}{0.0001} & \underline{3.772} & \textbf{0.362} & \underline{4.54} & \underline{0.281} &\textbf{0.175} &\underline{0.142} \\ 
& & &\multirow{1}{*}{0.001} & \textbf{3.784} & \textbf{0.362} & \textbf{4.554} & \textbf{0.278} &\textbf{0.175} &\textbf{0.14} \\ 
& & &\multirow{1}{*}{0.01} & 3.756 & \underline{0.361} & 4.521 & 0.284 &\underline{0.178} &0.146 \\ 
& & &\multirow{1}{*}{0.1} & 3.746 & 0.36 & 4.507 & 0.286 &0.18 &0.149 \\ 
& & &\multirow{1}{*}{0.5} & 3.748 & 0.36 & 4.52 & 0.285 &0.18 &0.146 \\ 
& & &\multirow{1}{*}{1} & 3.753 & 0.36 & 4.534 & 0.284 &0.18 &0.143 \\ 
& & &\multirow{1}{*}{2} & 3.704 & 0.357 & 4.492 & 0.294 &0.187 &0.151 \\ 
& & &\multirow{1}{*}{4} & 3.684 & 0.355 & 4.483 & 0.297 &0.191 &0.153 \\ 
\cmidrule{3-10}
& &\multirow{8}{*}{Coverage} & \multirow{1}{*}{0.0001} & 3.651 & \textbf{0.374} & 4.494 & \underline{0.304} &\textbf{0.148} &0.151 \\ 
& & &\multirow{1}{*}{0.001} & 3.633 & 0.372 & 4.468 & 0.307 &0.152 &0.156 \\ 
& & &\multirow{1}{*}{0.01} & 3.64 & \underline{0.373} & 4.478 & 0.306 &\underline{0.15} &0.154 \\ 
& & &\multirow{1}{*}{0.1} & \textbf{3.661} & \textbf{0.374} & \underline{4.504} & \textbf{0.302} &\textbf{0.148} &\underline{0.149} \\ 
& & &\multirow{1}{*}{0.5} & 3.637 & 0.372 & 4.479 & 0.306 &0.152 &0.154 \\ 
& & &\multirow{1}{*}{1} & 3.613 & 0.37 & 4.452 & 0.311 &0.157 &0.159 \\ 
& & &\multirow{1}{*}{2} & 3.64 & 0.372 & 4.488 & 0.306 &0.152 &0.152 \\ 
& & &\multirow{1}{*}{4} & \underline{3.659} & 0.372 & \textbf{4.529} & \textbf{0.302} &0.152 &\textbf{0.144} \\ 
\cmidrule{2-10}
& \multirow{16}{*}{40} & \multirow{8}{*}{Interacted distance} & \multirow{1}{*}{0.0001} & 5.245 & 0.441 & 6.298 & 0.308 &0.231 &0.172 \\ 
& & &\multirow{1}{*}{0.001} & 5.276 & 0.443 & 6.34 & 0.304 &0.228 &0.167 \\ 
& & &\multirow{1}{*}{0.01} & \underline{5.367} & \underline{0.447} & \underline{6.454} & \underline{0.292} &\underline{0.221} &\underline{0.152} \\ 
& & &\multirow{1}{*}{0.1} & 5.258 & 0.441 & 6.321 & 0.307 &0.231 &0.169 \\ 
& & &\multirow{1}{*}{0.5} & 5.29 & 0.443 & 6.367 & 0.302 &0.228 &0.163 \\ 
& & &\multirow{1}{*}{1} & \textbf{5.375} & \textbf{0.449} & \textbf{6.462} & \textbf{0.291} &\textbf{0.217} &\textbf{0.151} \\ 
& & &\multirow{1}{*}{2} & 5.247 & 0.441 & 6.332 & 0.308 &0.231 &0.168 \\ 
& & &\multirow{1}{*}{4} & 5.258 & 0.443 & 6.358 & 0.307 &0.228 &0.164 \\ 
\cmidrule{3-10}
& &\multirow{8}{*}{Coverage} & \multirow{1}{*}{0.0001} & \underline{5.129} & \textbf{0.476} & \underline{6.323} & \underline{0.324} &\textbf{0.17} &\underline{0.169} \\ 
& & &\multirow{1}{*}{0.001} & 5.06 & 0.472 & 6.233 & 0.333 &0.177 &0.181 \\ 
& & &\multirow{1}{*}{0.01} & 5.051 & 0.471 & 6.232 & 0.334 &0.179 &0.181 \\ 
& & &\multirow{1}{*}{0.1} & 5.079 & 0.472 & 6.276 & 0.33 &0.177 &0.175 \\ 
& & &\multirow{1}{*}{0.5} & 5.074 & 0.471 & 6.26 & 0.331 &0.179 &0.177 \\ 
& & &\multirow{1}{*}{1} & \textbf{5.137} & \underline{0.475} & \textbf{6.351} & \textbf{0.323} &\underline{0.172} &\textbf{0.165} \\ 
& & &\multirow{1}{*}{2} & 5.029 & 0.466 & 6.226 & 0.337 &0.188 &0.182 \\ 
& & &\multirow{1}{*}{4} & 5.01 & 0.462 & 6.222 & 0.339 &0.195 &0.182 \\ 

\end{tabular}}
\caption{Experiments over coat adopting jaccard distance in terms of genres. Results have been obtained by averaging 20 independent trails. Bold and underline values represent the best and second-best scores, respectively.}
\label{tab:jaccard_genres_coat_scores_table}
\end{table*}

==> coat/deterministic_jaccard_genres_scores_table.tex <==
\resizebox{\columnwidth}{!}{\begin{tabular}{c c c c c c c c c}
$k$ & $B$ & Strategy & \multicolumn{1}{c}{$D(C)$} & \multicolumn{1}{c}{$\textit{cov(C)}$} & \multicolumn{1}{c}{\textit{steps}} & \multicolumn{1}{c}{$\Delta_{\mathbbm{E[\textit{D}]}}$} & \multicolumn{1}{c}{$\Delta_{\mathbbm{E[\textit{cov}]}}$} &\multicolumn{1}{c}{$\Delta_{\mathbbm{E[\textit{steps}}]}$} \\  
\midrule
\multirow{21}{*}{2} & \multirow{7}{*}{10} & \multirow{1}{*}{Relevance} & 2.57 & 0.28 & 3.33 & 0.28 &0.17 &0.09 \\ 
\cmidrule{3-9}
& &\multirow{1}{*}{Interacted distance} & \textbf{2.84} & \textbf{0.31} & 3.32 & \textbf{0.2} &\textbf{0.08} &0.09 \\ 
& &\multirow{1}{*}{Coverage} & 2.74 & \textbf{0.31} & 3.32 & 0.23 &\textbf{0.08} &0.09 \\ 
\cmidrule{3-9}
& &\multirow{1}{*}{MMR} & 2.24 & 0.26 & 3.1 & 0.37 &0.23 &0.15 \\ 
& &\multirow{1}{*}{DUM} & 2.6 & 0.29 & 3.39 & 0.27 &0.14 &0.07 \\ 
& &\multirow{1}{*}{DPP} & 2.57 & 0.28 & 3.37 & 0.28 &0.17 &0.08 \\ 
& &\multirow{1}{*}{DGREC} & 2.04 & 0.24 & 3.01 & 0.43 &0.29 &0.18 \\ 
\cmidrule{2-9}
& \multirow{7}{*}{20} & \multirow{1}{*}{Relevance} & 3.64 & 0.35 & 4.78 & 0.31 &0.2 &0.1 \\ 
\cmidrule{3-9}
& &\multirow{1}{*}{Interacted distance} & \textbf{4.06} & 0.38 & 4.72 & \textbf{0.23} &0.13 &0.11 \\ 
& &\multirow{1}{*}{Coverage} & 3.85 & \textbf{0.4} & 4.72 & 0.27 &\textbf{0.09} &0.11 \\ 
\cmidrule{3-9}
& &\multirow{1}{*}{MMR} & 2.88 & 0.31 & 4.43 & 0.45 &0.29 &0.16 \\ 
& &\multirow{1}{*}{DUM} & 3.64 & 0.35 & 4.78 & 0.31 &0.2 &0.1 \\ 
& &\multirow{1}{*}{DPP} & 3.61 & 0.33 & 4.75 & 0.31 &0.25 &0.1 \\ 
& &\multirow{1}{*}{DGREC} & 3.01 & 0.3 & 4.31 & 0.43 &0.32 &0.19 \\ 
\cmidrule{2-9}
& \multirow{7}{*}{40} & \multirow{1}{*}{Relevance} & 5.16 & 0.41 & 6.9 & 0.32 &0.29 &0.09 \\ 
\cmidrule{3-9}
& &\multirow{1}{*}{Interacted distance} & \textbf{5.69} & 0.47 & 6.66 & \textbf{0.25} &0.18 &0.12 \\ 
& &\multirow{1}{*}{Coverage} & 5.31 & \textbf{0.51} & 6.62 & 0.3 &\textbf{0.11} &0.13 \\ 
\cmidrule{3-9}
& &\multirow{1}{*}{MMR} & 3.6 & 0.36 & 6.32 & 0.53 &0.37 &0.17 \\ 
& &\multirow{1}{*}{DUM} & 5.12 & 0.41 & 6.84 & 0.32 &0.29 &0.1 \\ 
& &\multirow{1}{*}{DPP} & 5.13 & 0.39 & 6.81 & 0.32 &0.32 &0.11 \\ 
& &\multirow{1}{*}{DGREC} & 4.37 & 0.37 & 6.18 & 0.42 &0.36 &0.19 \\ 
\midrule
\multirow{21}{*}{10} & \multirow{7}{*}{10} & \multirow{1}{*}{Relevance} & 2.35 & 0.26 & \textbf{3.32} & 0.34 &0.23 &\textbf{0.09} \\ 
\cmidrule{3-9}
& &\multirow{1}{*}{Interacted distance} & \textbf{2.65} & \textbf{0.29} & 3.21 & \textbf{0.26} &\textbf{0.14} &0.12 \\ 
& &\multirow{1}{*}{Coverage} & 2.57 & \textbf{0.29} & 3.17 & 0.28 &\textbf{0.14} &0.13 \\ 
\cmidrule{3-9}
& &\multirow{1}{*}{MMR} & 1.93 & 0.23 & 2.84 & 0.46 &0.32 &0.22 \\ 
& &\multirow{1}{*}{DUM} & 2.34 & 0.26 & \textbf{3.32} & 0.34 &0.23 &\textbf{0.09} \\ 
& &\multirow{1}{*}{DPP} & 2.47 & 0.27 & \textbf{3.32} & 0.31 &0.2 &\textbf{0.09} \\ 
& &\multirow{1}{*}{DGREC} & 1.71 & 0.22 & 2.62 & 0.52 &0.35 &0.28 \\ 
\cmidrule{2-9}
& \multirow{7}{*}{20} & \multirow{1}{*}{Relevance} & 3.44 & 0.32 & 4.73 & 0.34 &0.27 &0.11 \\ 
\cmidrule{3-9}
& &\multirow{1}{*}{Interacted distance} & 3.78 & 0.36 & 4.49 & 0.28 &0.18 &0.15 \\ 
& &\multirow{1}{*}{Coverage} & 3.72 & \textbf{0.38} & 4.53 & 0.29 &\textbf{0.13} &0.14 \\ 
\cmidrule{3-9}
& &\multirow{1}{*}{MMR} & 2.71 & 0.28 & 3.9 & 0.48 &0.36 &0.26 \\ 
& &\multirow{1}{*}{DUM} & 3.43 & 0.33 & 4.7 & 0.35 &0.25 &0.11 \\ 
& &\multirow{1}{*}{DPP} & 3.59 & 0.33 & 4.7 & 0.32 &0.25 &0.11 \\ 
& &\multirow{1}{*}{DGREC} & 2.51 & 0.27 & 3.64 & 0.52 &0.38 &0.31 \\ 
\cmidrule{2-9}
& \multirow{7}{*}{40} & \multirow{1}{*}{Relevance} & 4.94 & 0.39 & 6.73 & 0.35 &0.32 &0.12 \\ 
\cmidrule{3-9}
& &\multirow{1}{*}{Interacted distance} & \textbf{5.41} & 0.45 & 6.41 & \textbf{0.29} &0.22 &0.16 \\ 
& &\multirow{1}{*}{Coverage} & 5.09 & \textbf{0.48} & 6.24 & 0.33 &\textbf{0.16} &0.18 \\ 
\cmidrule{3-9}
& &\multirow{1}{*}{MMR} & 3.75 & 0.34 & 5.4 & 0.51 &0.41 &0.29 \\ 
& &\multirow{1}{*}{DUM} & 4.92 & 0.4 & 6.65 & 0.35 &0.3 &0.13 \\ 
& &\multirow{1}{*}{DPP} & 5.2 & 0.41 & 6.74 & 0.31 &0.29 &0.11 \\ 
& &\multirow{1}{*}{DGREC} & 3.6 & 0.33 & 5.11 & 0.53 &0.42 &0.33 \\ 
\midrule
\multirow{21}{*}{20} & \multirow{7}{*}{10} & \multirow{1}{*}{Relevance} & 2.42 & 0.27 & 3.35 & 0.32 &0.2 &0.08 \\ 
\cmidrule{3-9}
& &\multirow{1}{*}{Interacted distance} & \textbf{2.65} & \textbf{0.29} & 3.25 & \textbf{0.26} &\textbf{0.14} &0.11 \\ 
& &\multirow{1}{*}{Coverage} & 2.51 & \textbf{0.29} & 3.14 & 0.29 &\textbf{0.14} &0.14 \\ 
\cmidrule{3-9}
& &\multirow{1}{*}{MMR} & 1.98 & 0.24 & 2.86 & 0.44 &0.29 &0.22 \\ 
& &\multirow{1}{*}{DUM} & 2.44 & 0.27 & 3.33 & 0.31 &0.2 &0.09 \\ 
& &\multirow{1}{*}{DPP} & 2.51 & 0.27 & 3.31 & 0.29 &0.2 &0.1 \\ 
& &\multirow{1}{*}{DGREC} & 1.7 & 0.22 & 2.61 & 0.52 &0.35 &0.29 \\ 
\cmidrule{2-9}
& \multirow{7}{*}{20} & \multirow{1}{*}{Relevance} & 3.55 & 0.33 & 4.77 & 0.32 &0.25 &0.1 \\ 
\cmidrule{3-9}
& &\multirow{1}{*}{Interacted distance} & 3.75 & 0.36 & 4.52 & 0.28 &0.18 &0.15 \\ 
& &\multirow{1}{*}{Coverage} & 3.64 & \textbf{0.37} & 4.48 & 0.31 &\textbf{0.16} &0.15 \\ 
\cmidrule{3-9}
& &\multirow{1}{*}{MMR} & 2.8 & 0.29 & 3.94 & 0.47 &0.34 &0.26 \\ 
& &\multirow{1}{*}{DUM} & 3.61 & 0.34 & 4.8 & 0.31 &0.23 &0.09 \\ 
& &\multirow{1}{*}{DPP} & 3.68 & 0.34 & 4.74 & 0.3 &0.23 &0.1 \\ 
& &\multirow{1}{*}{DGREC} & 2.5 & 0.27 & 3.63 & 0.52 &0.38 &0.31 \\ 
\cmidrule{2-9}
& \multirow{7}{*}{40} & \multirow{1}{*}{Relevance} & 5.05 & 0.4 & 6.74 & 0.33 &0.3 &0.11 \\ 
\cmidrule{3-9}
& &\multirow{1}{*}{Interacted distance} & 5.29 & 0.44 & 6.37 & 0.3 &0.23 &0.16 \\ 
& &\multirow{1}{*}{Coverage} & 5.07 & \textbf{0.47} & 6.26 & 0.33 &\textbf{0.18} &0.18 \\ 
\cmidrule{3-9}
& &\multirow{1}{*}{MMR} & 3.82 & 0.35 & 5.36 & 0.5 &0.39 &0.3 \\ 
& &\multirow{1}{*}{DUM} & 5.19 & 0.42 & 6.84 & 0.32 &0.27 &0.1 \\ 
& &\multirow{1}{*}{DPP} & 5.33 & 0.42 & 6.8 & 0.3 &0.27 &0.11 \\ 
& &\multirow{1}{*}{DGREC} & 3.54 & 0.33 & 5.04 & 0.53 &0.42 &0.34 \\ 
\midrule
\end{tabular}}
\caption{Results on Coat. The best scores with a statistical significance $p<0.05$ are highlighted in bold.}
\label{tab:jaccard_genres_coat_scores_table}
 

==> coat/partial_scores_table.tex <==
\begin{table*}
 \centering 
\resizebox{0.6\textwidth}{!}{\begin{tabular}{c|c|c|c|c|c|c|c|c}
\hline 
k & Patience & Rec Strategy & \multicolumn{1}{c|}{$D(C)$} & \multicolumn{1}{c|}{$cov(C)$} & \multicolumn{1}{c|}{$steps$} &\multicolumn{1}{c|}{$\delta_R$} & \multicolumn{1}{c|}{$\delta_{cov}$} &\multicolumn{1}{c}{$\delta_{steps}$} \\ 
\hline\hline
\multirow{21}{*}{10} & \multirow{7}{*}{10} & \multirow{1}{*}{relevance} & 2.35 & 0.26 & \textbf{3.32} & 0.34 &0.23 &\textbf{0.09} \\ 
\cline{3-9}
& &\multirow{1}{*}{interacted distance w relevance} & \textbf{2.66} & \textbf{0.29} & \underline{3.22} & \textbf{0.25} &\textbf{0.14} &\underline{0.12} \\ 
& &\multirow{1}{*}{coverage w relevance} & \underline{2.54} & \textbf{0.29} & 3.13 & \underline{0.29} &\textbf{0.14} &0.14 \\ 
\cline{3-9}
& &\multirow{1}{*}{mmr} & 1.93 & 0.23 & 2.84 & 0.46 &0.32 &0.22 \\ 
& &\multirow{1}{*}{dpp} & 2.47 & \underline{0.27} & \textbf{3.32} & 0.31 &\underline{0.2} &\textbf{0.09} \\ 
& &\multirow{1}{*}{dum} & 2.34 & 0.26 & \textbf{3.32} & 0.34 &0.23 &\textbf{0.09} \\ 
& &\multirow{1}{*}{dgrec} & 1.71 & 0.22 & 2.62 & 0.52 &0.35 &0.28 \\ 
\hhline{~========}
& \multirow{7}{*}{20} & \multirow{1}{*}{relevance} & 3.44 & 0.32 & \textbf{4.73} & 0.34 &0.27 &\textbf{0.11} \\ 
\cline{3-9}
& &\multirow{1}{*}{interacted distance w relevance} & \textbf{3.8} & \underline{0.36} & 4.51 & \textbf{0.28} &\underline{0.18} &\underline{0.15} \\ 
& &\multirow{1}{*}{coverage w relevance} & \underline{3.68} & \textbf{0.38} & 4.48 & \underline{0.3} &\textbf{0.13} &\underline{0.15} \\ 
\cline{3-9}
& &\multirow{1}{*}{mmr} & 2.71 & 0.28 & 3.9 & 0.48 &0.36 &0.26 \\ 
& &\multirow{1}{*}{dpp} & 3.59 & 0.33 & \underline{4.7} & 0.32 &0.25 &\textbf{0.11} \\ 
& &\multirow{1}{*}{dum} & 3.43 & 0.33 & \underline{4.7} & 0.35 &0.25 &\textbf{0.11} \\ 
& &\multirow{1}{*}{dgrec} & 2.51 & 0.27 & 3.64 & 0.52 &0.38 &0.31 \\ 
\hhline{~========}
& \multirow{7}{*}{40} & \multirow{1}{*}{relevance} & 4.94 & 0.39 & \underline{6.73} & 0.35 &0.32 &\underline{0.12} \\ 
\cline{3-9}
& &\multirow{1}{*}{interacted distance w relevance} & \textbf{5.43} & \underline{0.45} & 6.43 & \textbf{0.28} &\underline{0.22} &0.16 \\ 
& &\multirow{1}{*}{coverage w relevance} & 5.11 & \textbf{0.48} & 6.26 & 0.33 &\textbf{0.16} &0.18 \\ 
\cline{3-9}
& &\multirow{1}{*}{mmr} & 3.75 & 0.34 & 5.4 & 0.51 &0.41 &0.29 \\ 
& &\multirow{1}{*}{dpp} & \underline{5.2} & 0.41 & \textbf{6.74} & \underline{0.31} &0.29 &\textbf{0.11} \\ 
& &\multirow{1}{*}{dum} & 4.92 & 0.4 & 6.65 & 0.35 &0.3 &0.13 \\ 
& &\multirow{1}{*}{dgrec} & 3.6 & 0.33 & 5.11 & 0.53 &0.42 &0.33 \\ 
\hline
\end{tabular}}
\caption{Experiments over coat adopting jaccard distance in terms of genres. Results have been obtained by averaging 20 independent trails. Bold and underline values represent the best and second-best scores, respectively.}
\label{tab:jaccard_genres_coat_scores_table}
\end{table*}

==> fig/toy_example.tex <==
\definecolor{bostonuniversityred}{rgb}{0.8, 0.0, 0.0}
\definecolor{ao_english}{rgb}{0.0, 0.5, 0.0}
\definecolor{cadmiumgreen}{rgb}{0.0, 0.42, 0.24}

\begin{figure}
\begin{adjustbox}{width=0.9\columnwidth, keepaspectratio, center}
\begin{tikzpicture}[
roundnode/.style={circle, draw=gray!60, fill=blue!5, very thick, minimum size=10mm},
squarenode/.style={rectangle, draw=gray!60, fill=green!5, very thick, minimum size=7mm},
diamondnode/.style={diamond, draw=gray!60, fill=red!5, very thick, minimum size=12mm, inner sep=1pt},
textnode/.style={rectangle, draw=black!0, minimum size=7mm}
]
%Nodes
\node[roundnode]      (user)                              {\textbf{U}};
\node[diamondnode]      (quits)       [below left=of user] {Quits};
\node[diamondnode]      (continues)       [below right=of user]{Goes};
\node[roundnode]      (relevance)       [below right=of quits] {\textbf{R}};
\node[squarenode]     (small)       [above=of quits] {Small $C$};
\node[textnode]           (low)         [above=of small] {\textcolor{bostonuniversityred}{\textbf{Lower Score}}};
{Keeps};
\node[squarenode]     (large)       [right=of continues] {Large $C$};
\node[roundnode]      (diversity)       [right=of large] {\textbf{D}};
\node[diamondnode]      (induces_1)       [above=of large]{Induce};
\node[diamondnode]      (induces_2)       [below=of large]{Induce};
\node[squarenode]     (homogeneous)       [right=of low] {Homogeneous $C$};
\node[squarenode]     (diverse)       [below left=of induces_2, yshift=0.5cm, xshift=-0.45cm] {Diverse $C$};
{Continues};
\node[textnode]           (high)         [left=of diverse, xshift=-0.3cm] {\textcolor{cadmiumgreen}{\textbf{Higher Score}}};
{Continues};

%Lines
\draw[-{Stealth[length=2mm, width=2mm]}] (user.south west) -- (quits.north east);
\draw[-{Stealth[length=2mm, width=2mm]}] (user.south east) -- (continues.north west);

\draw[-{Stealth[length=2mm, width=2mm]}] (relevance.north west) --  node [fill=white,anchor=center] {Low} (quits.south east) ;
\draw[-{Stealth[length=2mm, width=2mm]}] (relevance.north east) --  node [fill=white,anchor=center] {High} (continues.south west) ;
\draw[-{Stealth[length=2mm, width=2mm]}] (quits.north) -- (small.south) ;
\draw[-{Stealth[length=2mm, width=2mm]}] (small.north) -- (low.south) ;
\draw[-{Stealth[length=2mm, width=2mm]}] (continues.east) -- (large.west) ;
\draw[-{Stealth[length=2mm, width=2mm]}] (continues.east) -- (large.west) ;
\draw[-{Stealth[length=2mm, width=2mm]}] (diversity.north west) -- node [fill=white,anchor=center] {Low} (induces_1.south east) ;
\draw[-{Stealth[length=2mm, width=2mm]}] (diversity.south west) --  node [fill=white,anchor=center] {High}(induces_2.north east) ;
\draw[-{Stealth[length=2mm, width=2mm]}] (large.north) -- (induces_1.south) ;
\draw[-{Stealth[length=2mm, width=2mm]}] (large.south) -- (induces_2.north) ;
\draw[-{Stealth[length=2mm, width=2mm]}] (induces_1.north) |- (homogeneous.east) ;
\draw[-{Stealth[length=2mm, width=2mm]}] (induces_2.south) |- (diverse.east) ;
\draw[-{Stealth[length=2mm, width=2mm]}] (homogeneous.west) -- (low.east) ;
\draw[-{Stealth[length=2mm, width=2mm]}] (diverse.west) -- (high.east) ;
\end{tikzpicture}
\end{adjustbox}
\caption{Interplay induced in our simulation framework among \textit{relevance} (\textbf{R}), \textit{diversity} (\textbf{D}) and \textit{user behavior} (\textbf{U}).}
\label{fig:toy_example}
\end{figure}

==> movielens-1m/ali_alphas_table.tex <==
\begin{table*}
 \centering 
\resizebox{0.6\textwidth}{!}{\begin{tabular}{c c c c c c c c c c}
\midrule 
k & Patience & Rec Strategy  & $\alpha$ &  \multicolumn{1}{c}{R(C)} & \multicolumn{1}{c}{cov(C)} & \multicolumn{1}{c}{steps} &\multicolumn{1}{c}{$\delta_R$} & \multicolumn{1}{c}{$\delta_{cov}$} &\multicolumn{1}{c}{$\delta_{steps}$} \\ 
\midrule
\multirow{30}{*}{2} & \multirow{10}{*}{10} & \multirow{5}{*}{Interacted distance} & \multirow{1}{*}{-1} & 3.55 & \textbf{0.261} & 3.65 & 0.003 &\textbf{0.635} &0.003 \\ 
& & &\multirow{1}{*}{-0.5} & \textbf{3.558} & \textbf{0.261} & \textbf{3.66} & \textbf{0.001} &\textbf{0.635} &\textbf{0.0} \\ 
& & &\multirow{1}{*}{0} & 3.552 & \textbf{0.261} & 3.652 & \underline{0.002} &\textbf{0.635} &0.002 \\ 
& & &\multirow{1}{*}{0.5} & \underline{3.556} & \textbf{0.261} & \underline{3.657} & \textbf{0.001} &\textbf{0.635} &\underline{0.001} \\ 
& & &\multirow{1}{*}{1} & 2.466 & \underline{0.185} & 3.13 & 0.307 &\underline{0.741} &0.145 \\ 
\cmidrule{3-10}
& &\multirow{5}{*}{Coverage} & \multirow{1}{*}{-1} & \textbf{3.329} & \textbf{0.688} & \textbf{3.521} & \textbf{0.065} &\textbf{0.037} &\textbf{0.038} \\ 
& & &\multirow{1}{*}{-0.5} & \underline{3.324} & \textbf{0.688} & \underline{3.515} & \underline{0.066} &\textbf{0.037} &\underline{0.04} \\ 
& & &\multirow{1}{*}{0} & 3.316 & \textbf{0.688} & 3.509 & 0.069 &\textbf{0.037} &0.041 \\ 
& & &\multirow{1}{*}{0.5} & 3.319 & \textbf{0.688} & 3.513 & 0.068 &\textbf{0.037} &\underline{0.04} \\ 
& & &\multirow{1}{*}{1} & 0.186 & \underline{0.075} & 2.705 & 0.948 &\underline{0.895} &0.261 \\ 
\cmidrule{2-10}
& \multirow{10}{*}{20} & \multirow{5}{*}{Interacted distance} & \multirow{1}{*}{-1} & \underline{5.224} & \textbf{0.372} & \underline{5.274} & \underline{0.004} &\textbf{0.55} &\underline{0.004} \\ 
& & &\multirow{1}{*}{-0.5} & \textbf{5.227} & \textbf{0.372} & \textbf{5.276} & \textbf{0.003} &\textbf{0.55} &\textbf{0.003} \\ 
& & &\multirow{1}{*}{0} & 5.221 & \textbf{0.372} & 5.271 & \underline{0.004} &\textbf{0.55} &\underline{0.004} \\ 
& & &\multirow{1}{*}{0.5} & 5.223 & \textbf{0.372} & 5.273 & \underline{0.004} &\textbf{0.55} &\underline{0.004} \\ 
& & &\multirow{1}{*}{1} & 3.475 & \underline{0.238} & 4.397 & 0.337 &\underline{0.712} &0.169 \\ 
\cmidrule{3-10}
& &\multirow{5}{*}{Coverage} & \multirow{1}{*}{-1} & \underline{4.886} & \underline{0.804} & \underline{5.124} & \underline{0.068} &\underline{0.027} &\underline{0.032} \\ 
& & &\multirow{1}{*}{-0.5} & \textbf{4.891} & \textbf{0.805} & \textbf{5.128} & \textbf{0.067} &\textbf{0.025} &\textbf{0.031} \\ 
& & &\multirow{1}{*}{0} & 4.879 & \textbf{0.805} & 5.115 & 0.07 &\textbf{0.025} &0.034 \\ 
& & &\multirow{1}{*}{0.5} & 4.864 & \underline{0.804} & 5.101 & 0.072 &\underline{0.027} &0.036 \\ 
& & &\multirow{1}{*}{1} & 0.354 & 0.086 & 3.846 & 0.932 &0.896 &0.273 \\ 
\cmidrule{2-10}
& \multirow{10}{*}{40} & \multirow{5}{*}{Interacted distance} & \multirow{1}{*}{-1} & \textbf{7.516} & \textbf{0.517} & \textbf{7.548} & \textbf{0.009} &\textbf{0.428} &\textbf{0.008} \\ 
& & &\multirow{1}{*}{-0.5} & 7.499 & \textbf{0.517} & 7.531 & 0.011 &\textbf{0.428} &0.01 \\ 
& & &\multirow{1}{*}{0} & \underline{7.509} & \textbf{0.517} & \underline{7.539} & \underline{0.01} &\textbf{0.428} &\underline{0.009} \\ 
& & &\multirow{1}{*}{0.5} & 7.494 & \underline{0.516} & 7.526 & 0.012 &\underline{0.429} &0.011 \\ 
& & &\multirow{1}{*}{1} & 4.782 & 0.303 & 6.178 & 0.369 &0.665 &0.188 \\ 
\cmidrule{3-10}
& &\multirow{5}{*}{Coverage} & \multirow{1}{*}{-1} & 6.959 & \textbf{0.89} & 7.443 & \underline{0.082} &\textbf{0.015} &0.022 \\ 
& & &\multirow{1}{*}{-0.5} & \textbf{6.969} & \textbf{0.89} & \textbf{7.456} & \textbf{0.081} &\textbf{0.015} &\textbf{0.02} \\ 
& & &\multirow{1}{*}{0} & 6.943 & \underline{0.889} & 7.425 & 0.085 &\underline{0.016} &0.024 \\ 
& & &\multirow{1}{*}{0.5} & \underline{6.965} & \textbf{0.89} & \underline{7.452} & \underline{0.082} &\textbf{0.015} &\underline{0.021} \\ 
& & &\multirow{1}{*}{1} & 0.685 & 0.101 & 5.482 & 0.91 &0.888 &0.28 \\ 
\midrule
\multirow{30}{*}{10} & \multirow{10}{*}{10} & \multirow{5}{*}{Interacted distance} & \multirow{1}{*}{-1} & \underline{3.556} & \textbf{0.264} & \underline{3.656} & \underline{0.001} &\textbf{0.631} &\underline{0.001} \\ 
& & &\multirow{1}{*}{-0.5} & \textbf{3.561} & \textbf{0.264} & \textbf{3.661} & \textbf{-0.0} &\textbf{0.631} &\textbf{-0.0} \\ 
& & &\multirow{1}{*}{0} & 3.548 & \underline{0.263} & 3.649 & 0.003 &\underline{0.632} &0.003 \\ 
& & &\multirow{1}{*}{0.5} & 3.554 & \underline{0.263} & 3.654 & 0.002 &\underline{0.632} &0.002 \\ 
& & &\multirow{1}{*}{1} & 2.428 & 0.186 & 2.802 & 0.318 &0.74 &0.234 \\ 
\cmidrule{3-10}
& &\multirow{5}{*}{Coverage} & \multirow{1}{*}{-1} & \underline{3.236} & 0.635 & \underline{3.465} & \underline{0.091} &0.112 &\underline{0.053} \\ 
& & &\multirow{1}{*}{-0.5} & 3.228 & 0.635 & 3.458 & 0.093 &0.112 &0.055 \\ 
& & &\multirow{1}{*}{0} & 3.229 & \underline{0.637} & 3.458 & 0.093 &\underline{0.109} &0.055 \\ 
& & &\multirow{1}{*}{0.5} & \textbf{3.241} & \textbf{0.639} & \textbf{3.471} & \textbf{0.09} &\textbf{0.106} &\textbf{0.052} \\ 
& & &\multirow{1}{*}{1} & 0.266 & 0.089 & 1.464 & 0.925 &0.875 &0.6 \\ 
\cmidrule{2-10}
& \multirow{10}{*}{20} & \multirow{5}{*}{Interacted distance} & \multirow{1}{*}{-1} & \underline{5.241} & \underline{0.378} & \textbf{5.291} & \textbf{0.0} &\underline{0.542} &\textbf{0.0} \\ 
& & &\multirow{1}{*}{-0.5} & 5.239 & \textbf{0.379} & \underline{5.289} & \underline{0.001} &\textbf{0.541} &\underline{0.001} \\ 
& & &\multirow{1}{*}{0} & \textbf{5.242} & \textbf{0.379} & \textbf{5.291} & \textbf{0.0} &\textbf{0.541} &\textbf{0.0} \\ 
& & &\multirow{1}{*}{0.5} & 5.237 & \underline{0.378} & 5.288 & \underline{0.001} &\underline{0.542} &\underline{0.001} \\ 
& & &\multirow{1}{*}{1} & 3.269 & 0.234 & 3.693 & 0.377 &0.717 &0.302 \\ 
\cmidrule{3-10}
& &\multirow{5}{*}{Coverage} & \multirow{1}{*}{-1} & 4.777 & 0.759 & 5.037 & \underline{0.089} &0.081 &0.048 \\ 
& & &\multirow{1}{*}{-0.5} & 4.779 & \underline{0.76} & 5.04 & \underline{0.089} &\underline{0.08} &0.048 \\ 
& & &\multirow{1}{*}{0} & \textbf{4.79} & \textbf{0.762} & \textbf{5.049} & \textbf{0.087} &\textbf{0.077} &\textbf{0.046} \\ 
& & &\multirow{1}{*}{0.5} & \underline{4.785} & \textbf{0.762} & \underline{5.045} & \textbf{0.087} &\textbf{0.077} &\underline{0.047} \\ 
& & &\multirow{1}{*}{1} & 0.377 & 0.099 & 1.93 & 0.928 &0.88 &0.635 \\ 
\cmidrule{2-10}
& \multirow{10}{*}{40} & \multirow{5}{*}{Interacted distance} & \multirow{1}{*}{-1} & \underline{7.515} & \textbf{0.525} & \underline{7.552} & \underline{0.009} &\textbf{0.419} &\underline{0.008} \\ 
& & &\multirow{1}{*}{-0.5} & \textbf{7.524} & \textbf{0.525} & \textbf{7.559} & \textbf{0.008} &\textbf{0.419} &\textbf{0.007} \\ 
& & &\multirow{1}{*}{0} & 7.509 & \underline{0.524} & 7.545 & 0.01 &\underline{0.42} &\underline{0.008} \\ 
& & &\multirow{1}{*}{0.5} & 7.503 & \underline{0.524} & 7.539 & 0.011 &\underline{0.42} &0.009 \\ 
& & &\multirow{1}{*}{1} & 4.317 & 0.292 & 4.885 & 0.431 &0.677 &0.358 \\ 
\cmidrule{3-10}
& &\multirow{5}{*}{Coverage} & \multirow{1}{*}{-1} & 6.849 & 0.857 & 7.316 & 0.097 &0.051 &0.039 \\ 
& & &\multirow{1}{*}{-0.5} & \underline{6.859} & \underline{0.858} & \underline{7.327} & \underline{0.096} &\underline{0.05} &\textbf{0.037} \\ 
& & &\multirow{1}{*}{0} & 6.854 & \underline{0.858} & 7.323 & \underline{0.096} &\underline{0.05} &\underline{0.038} \\ 
& & &\multirow{1}{*}{0.5} & \textbf{6.86} & \textbf{0.86} & \textbf{7.33} & \textbf{0.095} &\textbf{0.048} &\textbf{0.037} \\ 
& & &\multirow{1}{*}{1} & 0.525 & 0.109 & 2.618 & 0.931 &0.879 &0.656 \\ 
\midrule
\multirow{30}{*}{20} & \multirow{10}{*}{10} & \multirow{5}{*}{Interacted distance} & \multirow{1}{*}{-1} & \underline{3.559} & \underline{0.267} & \underline{3.658} & \underline{0.0} &\underline{0.626} &\underline{0.001} \\ 
& & &\multirow{1}{*}{-0.5} & 3.556 & \underline{0.267} & 3.656 & 0.001 &\underline{0.626} &\underline{0.001} \\ 
& & &\multirow{1}{*}{0} & 3.551 & \underline{0.267} & 3.652 & 0.003 &\underline{0.626} &0.002 \\ 
& & &\multirow{1}{*}{0.5} & \textbf{3.565} & \textbf{0.268} & \textbf{3.664} & \textbf{-0.001} &\textbf{0.625} &\textbf{-0.001} \\ 
& & &\multirow{1}{*}{1} & 2.435 & 0.187 & 2.798 & 0.316 &0.738 &0.236 \\ 
\cmidrule{3-10}
& &\multirow{5}{*}{Coverage} & \multirow{1}{*}{-1} & 3.209 & 0.607 & 3.452 & 0.099 &0.151 &0.057 \\ 
& & &\multirow{1}{*}{-0.5} & 3.215 & 0.609 & 3.458 & 0.097 &0.148 &0.055 \\ 
& & &\multirow{1}{*}{0} & \underline{3.221} & \underline{0.611} & \underline{3.464} & \underline{0.095} &\underline{0.145} &\underline{0.054} \\ 
& & &\multirow{1}{*}{0.5} & \textbf{3.228} & \textbf{0.613} & \textbf{3.47} & \textbf{0.093} &\textbf{0.142} &\textbf{0.052} \\ 
& & &\multirow{1}{*}{1} & 0.311 & 0.093 & 1.259 & 0.913 &0.87 &0.656 \\ 
\cmidrule{2-10}
& \multirow{10}{*}{20} & \multirow{5}{*}{Interacted distance} & \multirow{1}{*}{-1} & 5.225 & \underline{0.383} & 5.277 & 0.004 &\underline{0.536} &0.003 \\ 
& & &\multirow{1}{*}{-0.5} & 5.23 & \textbf{0.385} & 5.282 & 0.003 &\textbf{0.534} &0.002 \\ 
& & &\multirow{1}{*}{0} & \textbf{5.246} & \textbf{0.385} & \textbf{5.297} & \textbf{-0.0} &\textbf{0.534} &\textbf{-0.001} \\ 
& & &\multirow{1}{*}{0.5} & \underline{5.239} & \textbf{0.385} & \underline{5.291} & \underline{0.001} &\textbf{0.534} &\underline{0.0} \\ 
& & &\multirow{1}{*}{1} & 3.272 & 0.236 & 3.666 & 0.376 &0.714 &0.307 \\ 
\cmidrule{3-10}
& &\multirow{5}{*}{Coverage} & \multirow{1}{*}{-1} & \textbf{4.758} & 0.735 & \textbf{5.025} & \textbf{0.093} &0.11 &\textbf{0.051} \\ 
& & &\multirow{1}{*}{-0.5} & \underline{4.756} & \underline{0.736} & \underline{5.024} & \textbf{0.093} &\underline{0.109} &\textbf{0.051} \\ 
& & &\multirow{1}{*}{0} & 4.744 & \underline{0.736} & 5.012 & \underline{0.095} &\underline{0.109} &\underline{0.053} \\ 
& & &\multirow{1}{*}{0.5} & 4.747 & \textbf{0.737} & 5.013 & \underline{0.095} &\textbf{0.108} &\underline{0.053} \\ 
& & &\multirow{1}{*}{1} & 0.448 & 0.109 & 1.553 & 0.915 &0.868 &0.707 \\ 
\cmidrule{2-10}
& \multirow{10}{*}{40} & \multirow{5}{*}{Interacted distance} & \multirow{1}{*}{-1} & 7.518 & 0.531 & 7.56 & 0.009 &0.412 &\underline{0.006} \\ 
& & &\multirow{1}{*}{-0.5} & 7.526 & \underline{0.532} & \underline{7.569} & \underline{0.008} &\underline{0.411} &\textbf{0.005} \\ 
& & &\multirow{1}{*}{0} & \textbf{7.53} & \underline{0.532} & \textbf{7.572} & \textbf{0.007} &\underline{0.411} &\textbf{0.005} \\ 
& & &\multirow{1}{*}{0.5} & \underline{7.528} & \textbf{0.533} & \textbf{7.572} & \textbf{0.007} &\textbf{0.41} &\textbf{0.005} \\ 
& & &\multirow{1}{*}{1} & 4.303 & 0.294 & 4.805 & 0.433 &0.674 &0.369 \\ 
\cmidrule{3-10}
& &\multirow{5}{*}{Coverage} & \multirow{1}{*}{-1} & 6.829 & 0.838 & 7.286 & 0.1 &0.072 &\underline{0.042} \\ 
& & &\multirow{1}{*}{-0.5} & \textbf{6.838} & \underline{0.84} & \textbf{7.296} & \textbf{0.098} &\underline{0.07} &\textbf{0.041} \\ 
& & &\multirow{1}{*}{0} & \underline{6.83} & \textbf{0.841} & \underline{7.288} & \underline{0.099} &\textbf{0.069} &\underline{0.042} \\ 
& & &\multirow{1}{*}{0.5} & 6.826 & \textbf{0.841} & 7.284 & 0.1 &\textbf{0.069} &0.043 \\ 
& & &\multirow{1}{*}{1} & 0.617 & 0.126 & 2.016 & 0.919 &0.86 &0.735 \\ 

\end{tabular}}
\caption{Experiments over movielens-1m adopting jaccard distance in terms of genres. Results have been obtained by averaging 20 independent trails. Bold and underline values represent the best and second-best scores, respectively.}
\label{tab:jaccard_genres_movielens-1m_scores_table}
\end{table*}

==> movielens-1m/clayton_alphas_table.tex <==
\begin{table*}
 \centering 
\resizebox{0.6\textwidth}{!}{\begin{tabular}{c c c c c c c c c c}
\midrule 
k & Patience & Rec Strategy  & $\alpha$ &  \multicolumn{1}{c}{R(C)} & \multicolumn{1}{c}{cov(C)} & \multicolumn{1}{c}{steps} &\multicolumn{1}{c}{$\delta_R$} & \multicolumn{1}{c}{$\delta_{cov}$} &\multicolumn{1}{c}{$\delta_{steps}$} \\ 
\midrule
\multirow{48}{*}{2} & \multirow{16}{*}{10} & \multirow{8}{*}{Interacted distance} & \multirow{1}{*}{0.0001} & 3.557 & \underline{0.261} & 3.657 & 0.001 &\underline{0.635} &0.001 \\ 
& & &\multirow{1}{*}{0.001} & 3.559 & \underline{0.261} & 3.659 & 0.0 &\underline{0.635} &\underline{0.0} \\ 
& & &\multirow{1}{*}{0.01} & \underline{3.562} & \textbf{0.262} & 3.66 & \underline{-0.001} &\textbf{0.633} &\underline{0.0} \\ 
& & &\multirow{1}{*}{0.1} & 3.559 & \underline{0.261} & \underline{3.661} & 0.0 &\underline{0.635} &\underline{-0.0} \\ 
& & &\multirow{1}{*}{0.5} & 3.547 & 0.26 & 3.648 & 0.004 &0.636 &0.003 \\ 
& & &\multirow{1}{*}{1} & 3.557 & \underline{0.261} & 3.656 & 0.001 &\underline{0.635} &0.001 \\ 
& & &\multirow{1}{*}{2} & 3.551 & \underline{0.261} & 3.651 & 0.003 &\underline{0.635} &0.003 \\ 
& & &\multirow{1}{*}{4} & \textbf{3.567} & \textbf{0.262} & \textbf{3.665} & \textbf{-0.002} &\textbf{0.633} &\textbf{-0.001} \\ 
\cmidrule{3-10}
& &\multirow{8}{*}{Coverage} & \multirow{1}{*}{0.0001} & 3.318 & \textbf{0.688} & 3.51 & \underline{0.068} &\textbf{0.037} &\underline{0.041} \\ 
& & &\multirow{1}{*}{0.001} & \textbf{3.321} & \textbf{0.688} & \textbf{3.514} & \textbf{0.067} &\textbf{0.037} &\textbf{0.04} \\ 
& & &\multirow{1}{*}{0.01} & 3.312 & \underline{0.687} & 3.505 & 0.07 &\underline{0.039} &0.042 \\ 
& & &\multirow{1}{*}{0.1} & 3.319 & \textbf{0.688} & \underline{3.512} & \underline{0.068} &\textbf{0.037} &\textbf{0.04} \\ 
& & &\multirow{1}{*}{0.5} & 3.314 & \textbf{0.688} & 3.507 & 0.069 &\textbf{0.037} &0.042 \\ 
& & &\multirow{1}{*}{1} & \underline{3.32} & \textbf{0.688} & \underline{3.512} & \textbf{0.067} &\textbf{0.037} &\textbf{0.04} \\ 
& & &\multirow{1}{*}{2} & \textbf{3.321} & \textbf{0.688} & \textbf{3.514} & \textbf{0.067} &\textbf{0.037} &\textbf{0.04} \\ 
& & &\multirow{1}{*}{4} & \underline{3.32} & 0.686 & \textbf{3.514} & \textbf{0.067} &0.04 &\textbf{0.04} \\ 
\cmidrule{2-10}
& \multirow{16}{*}{20} & \multirow{8}{*}{Interacted distance} & \multirow{1}{*}{0.0001} & 5.226 & \underline{0.372} & 5.277 & \underline{0.003} &\underline{0.55} &\underline{0.003} \\ 
& & &\multirow{1}{*}{0.001} & 5.223 & \underline{0.372} & 5.272 & 0.004 &\underline{0.55} &0.004 \\ 
& & &\multirow{1}{*}{0.01} & \textbf{5.231} & \textbf{0.373} & \textbf{5.282} & \textbf{0.002} &\textbf{0.548} &\textbf{0.002} \\ 
& & &\multirow{1}{*}{0.1} & 5.212 & \underline{0.372} & 5.263 & 0.006 &\underline{0.55} &0.006 \\ 
& & &\multirow{1}{*}{0.5} & 5.229 & \textbf{0.373} & 5.279 & \underline{0.003} &\textbf{0.548} &\underline{0.003} \\ 
& & &\multirow{1}{*}{1} & 5.228 & \textbf{0.373} & 5.278 & \underline{0.003} &\textbf{0.548} &\underline{0.003} \\ 
& & &\multirow{1}{*}{2} & \underline{5.23} & \textbf{0.373} & \underline{5.28} & \underline{0.003} &\textbf{0.548} &\underline{0.003} \\ 
& & &\multirow{1}{*}{4} & 5.229 & \textbf{0.373} & \underline{5.28} & \underline{0.003} &\textbf{0.548} &\underline{0.003} \\ 
\cmidrule{3-10}
& &\multirow{8}{*}{Coverage} & \multirow{1}{*}{0.0001} & \underline{4.898} & \textbf{0.806} & \underline{5.136} & \underline{0.066} &\textbf{0.024} &\underline{0.03} \\ 
& & &\multirow{1}{*}{0.001} & 4.879 & 0.804 & 5.116 & 0.07 &0.027 &0.034 \\ 
& & &\multirow{1}{*}{0.01} & \textbf{4.902} & \textbf{0.806} & \textbf{5.138} & \textbf{0.065} &\textbf{0.024} &\textbf{0.029} \\ 
& & &\multirow{1}{*}{0.1} & 4.892 & \underline{0.805} & 5.13 & 0.067 &\underline{0.025} &0.031 \\ 
& & &\multirow{1}{*}{0.5} & 4.89 & \underline{0.805} & 5.128 & 0.067 &\underline{0.025} &0.031 \\ 
& & &\multirow{1}{*}{1} & 4.885 & \underline{0.805} & 5.124 & 0.068 &\underline{0.025} &0.032 \\ 
& & &\multirow{1}{*}{2} & 4.896 & \underline{0.805} & 5.135 & \underline{0.066} &\underline{0.025} &\underline{0.03} \\ 
& & &\multirow{1}{*}{4} & 4.885 & 0.804 & 5.123 & 0.068 &0.027 &0.032 \\ 
\cmidrule{2-10}
& \multirow{16}{*}{40} & \multirow{8}{*}{Interacted distance} & \multirow{1}{*}{0.0001} & \underline{7.511} & \underline{0.517} & \underline{7.542} & \underline{0.01} &\underline{0.428} &\underline{0.009} \\ 
& & &\multirow{1}{*}{0.001} & 7.505 & \underline{0.517} & 7.537 & \underline{0.01} &\underline{0.428} &\underline{0.009} \\ 
& & &\multirow{1}{*}{0.01} & 7.507 & \underline{0.517} & 7.537 & \underline{0.01} &\underline{0.428} &\underline{0.009} \\ 
& & &\multirow{1}{*}{0.1} & \underline{7.511} & \textbf{0.518} & 7.541 & \underline{0.01} &\textbf{0.426} &\underline{0.009} \\ 
& & &\multirow{1}{*}{0.5} & 7.51 & \underline{0.517} & 7.54 & \underline{0.01} &\underline{0.428} &\underline{0.009} \\ 
& & &\multirow{1}{*}{1} & 7.507 & \textbf{0.518} & 7.54 & \underline{0.01} &\textbf{0.426} &\underline{0.009} \\ 
& & &\multirow{1}{*}{2} & \textbf{7.514} & \textbf{0.518} & \textbf{7.545} & \textbf{0.009} &\textbf{0.426} &\textbf{0.008} \\ 
& & &\multirow{1}{*}{4} & 7.499 & \underline{0.517} & 7.531 & 0.011 &\underline{0.428} &0.01 \\ 
\cmidrule{3-10}
& &\multirow{8}{*}{Coverage} & \multirow{1}{*}{0.0001} & 6.953 & \underline{0.889} & 7.438 & 0.083 &\underline{0.016} &0.022 \\ 
& & &\multirow{1}{*}{0.001} & 6.96 & \textbf{0.89} & 7.446 & \underline{0.082} &\textbf{0.015} &\underline{0.021} \\ 
& & &\multirow{1}{*}{0.01} & 6.945 & \underline{0.889} & 7.429 & 0.084 &\underline{0.016} &0.024 \\ 
& & &\multirow{1}{*}{0.1} & 6.955 & \underline{0.889} & 7.44 & 0.083 &\underline{0.016} &0.022 \\ 
& & &\multirow{1}{*}{0.5} & 6.955 & \underline{0.889} & 7.44 & 0.083 &\underline{0.016} &0.022 \\ 
& & &\multirow{1}{*}{1} & \underline{6.968} & \textbf{0.89} & \underline{7.454} & \textbf{0.081} &\textbf{0.015} &\textbf{0.02} \\ 
& & &\multirow{1}{*}{2} & \textbf{6.97} & \underline{0.889} & \textbf{7.456} & \textbf{0.081} &\underline{0.016} &\textbf{0.02} \\ 
& & &\multirow{1}{*}{4} & 6.958 & 0.888 & 7.444 & 0.083 &0.017 &0.022 \\ 
\midrule
\multirow{48}{*}{10} & \multirow{16}{*}{10} & \multirow{8}{*}{Interacted distance} & \multirow{1}{*}{0.0001} & 3.555 & \textbf{0.264} & 3.656 & \underline{0.001} &\textbf{0.631} &\underline{0.001} \\ 
& & &\multirow{1}{*}{0.001} & 3.556 & \textbf{0.264} & 3.655 & \underline{0.001} &\textbf{0.631} &\underline{0.001} \\ 
& & &\multirow{1}{*}{0.01} & \textbf{3.561} & \textbf{0.264} & \textbf{3.661} & \textbf{-0.0} &\textbf{0.631} &\textbf{-0.0} \\ 
& & &\multirow{1}{*}{0.1} & 3.555 & \textbf{0.264} & 3.656 & \underline{0.001} &\textbf{0.631} &\underline{0.001} \\ 
& & &\multirow{1}{*}{0.5} & \underline{3.56} & \textbf{0.264} & \underline{3.66} & \textbf{0.0} &\textbf{0.631} &\textbf{0.0} \\ 
& & &\multirow{1}{*}{1} & 3.554 & \underline{0.263} & 3.655 & 0.002 &\underline{0.632} &\underline{0.001} \\ 
& & &\multirow{1}{*}{2} & 3.55 & \underline{0.263} & 3.651 & 0.003 &\underline{0.632} &0.003 \\ 
& & &\multirow{1}{*}{4} & 3.551 & \underline{0.263} & 3.652 & 0.003 &\underline{0.632} &0.002 \\ 
\cmidrule{3-10}
& &\multirow{8}{*}{Coverage} & \multirow{1}{*}{0.0001} & 3.232 & 0.637 & 3.463 & 0.092 &0.109 &0.054 \\ 
& & &\multirow{1}{*}{0.001} & 3.238 & 0.638 & 3.468 & 0.091 &0.107 &0.053 \\ 
& & &\multirow{1}{*}{0.01} & 3.229 & 0.637 & 3.459 & 0.093 &0.109 &0.055 \\ 
& & &\multirow{1}{*}{0.1} & \underline{3.241} & 0.638 & \underline{3.471} & \underline{0.09} &0.107 &\underline{0.052} \\ 
& & &\multirow{1}{*}{0.5} & 3.237 & 0.639 & 3.466 & 0.091 &0.106 &0.053 \\ 
& & &\multirow{1}{*}{1} & 3.234 & 0.639 & 3.464 & 0.092 &0.106 &0.054 \\ 
& & &\multirow{1}{*}{2} & \textbf{3.254} & \textbf{0.642} & \textbf{3.484} & \textbf{0.086} &\textbf{0.102} &\textbf{0.048} \\ 
& & &\multirow{1}{*}{4} & 3.235 & \underline{0.641} & 3.466 & 0.091 &\underline{0.103} &0.053 \\ 
\cmidrule{2-10}
& \multirow{16}{*}{20} & \multirow{8}{*}{Interacted distance} & \multirow{1}{*}{0.0001} & 5.239 & \textbf{0.379} & 5.29 & \underline{0.001} &\textbf{0.541} &0.001 \\ 
& & &\multirow{1}{*}{0.001} & \underline{5.242} & \textbf{0.379} & \underline{5.293} & \textbf{0.0} &\textbf{0.541} &\underline{0.0} \\ 
& & &\multirow{1}{*}{0.01} & 5.227 & \underline{0.378} & 5.278 & 0.003 &\underline{0.542} &0.003 \\ 
& & &\multirow{1}{*}{0.1} & 5.228 & \underline{0.378} & 5.28 & 0.003 &\underline{0.542} &0.003 \\ 
& & &\multirow{1}{*}{0.5} & 5.237 & \underline{0.378} & 5.288 & \underline{0.001} &\underline{0.542} &0.001 \\ 
& & &\multirow{1}{*}{1} & 5.232 & \underline{0.378} & 5.283 & 0.002 &\underline{0.542} &0.002 \\ 
& & &\multirow{1}{*}{2} & \textbf{5.246} & \textbf{0.379} & \textbf{5.297} & \textbf{-0.0} &\textbf{0.541} &\textbf{-0.001} \\ 
& & &\multirow{1}{*}{4} & 5.217 & 0.377 & 5.268 & 0.005 &0.544 &0.005 \\ 
\cmidrule{3-10}
& &\multirow{8}{*}{Coverage} & \multirow{1}{*}{0.0001} & 4.77 & 0.761 & 5.03 & 0.09 &0.079 &0.05 \\ 
& & &\multirow{1}{*}{0.001} & \underline{4.784} & 0.762 & 5.042 & \underline{0.088} &0.077 &0.048 \\ 
& & &\multirow{1}{*}{0.01} & 4.783 & 0.762 & 5.043 & \underline{0.088} &0.077 &\underline{0.047} \\ 
& & &\multirow{1}{*}{0.1} & 4.778 & 0.762 & 5.037 & 0.089 &0.077 &0.048 \\ 
& & &\multirow{1}{*}{0.5} & \underline{4.784} & 0.762 & 5.043 & \underline{0.088} &0.077 &\underline{0.047} \\ 
& & &\multirow{1}{*}{1} & 4.782 & 0.763 & 5.043 & \underline{0.088} &0.076 &\underline{0.047} \\ 
& & &\multirow{1}{*}{2} & \textbf{4.789} & \underline{0.764} & \underline{5.048} & \textbf{0.087} &\underline{0.075} &\textbf{0.046} \\ 
& & &\multirow{1}{*}{4} & \textbf{4.789} & \textbf{0.765} & \textbf{5.05} & \textbf{0.087} &\textbf{0.074} &\textbf{0.046} \\ 
\cmidrule{2-10}
& \multirow{16}{*}{40} & \multirow{8}{*}{Interacted distance} & \multirow{1}{*}{0.0001} & \textbf{7.538} & \textbf{0.527} & \textbf{7.573} & \textbf{0.006} &\textbf{0.416} &\textbf{0.005} \\ 
& & &\multirow{1}{*}{0.001} & \underline{7.535} & \underline{0.525} & \underline{7.571} & \textbf{0.006} &\underline{0.419} &\textbf{0.005} \\ 
& & &\multirow{1}{*}{0.01} & 7.515 & 0.524 & 7.552 & 0.009 &0.42 &0.008 \\ 
& & &\multirow{1}{*}{0.1} & 7.509 & 0.524 & 7.545 & 0.01 &0.42 &0.008 \\ 
& & &\multirow{1}{*}{0.5} & 7.512 & 0.524 & 7.548 & 0.01 &0.42 &0.008 \\ 
& & &\multirow{1}{*}{1} & 7.509 & 0.524 & 7.545 & 0.01 &0.42 &0.008 \\ 
& & &\multirow{1}{*}{2} & 7.52 & \underline{0.525} & 7.557 & \underline{0.008} &\underline{0.419} &\underline{0.007} \\ 
& & &\multirow{1}{*}{4} & 7.516 & \underline{0.525} & 7.553 & 0.009 &\underline{0.419} &\underline{0.007} \\ 
\cmidrule{3-10}
& &\multirow{8}{*}{Coverage} & \multirow{1}{*}{0.0001} & 6.858 & 0.859 & 7.328 & 0.096 &0.049 &0.037 \\ 
& & &\multirow{1}{*}{0.001} & 6.833 & 0.858 & 7.297 & 0.099 &0.05 &0.041 \\ 
& & &\multirow{1}{*}{0.01} & 6.87 & 0.859 & 7.339 & \underline{0.094} &0.049 &\underline{0.035} \\ 
& & &\multirow{1}{*}{0.1} & 6.847 & 0.858 & 7.316 & 0.097 &0.05 &0.039 \\ 
& & &\multirow{1}{*}{0.5} & 6.852 & 0.859 & 7.321 & 0.097 &0.049 &0.038 \\ 
& & &\multirow{1}{*}{1} & 6.85 & 0.859 & 7.319 & 0.097 &0.049 &0.038 \\ 
& & &\multirow{1}{*}{2} & \underline{6.873} & \underline{0.86} & \underline{7.345} & \underline{0.094} &\underline{0.048} &\underline{0.035} \\ 
& & &\multirow{1}{*}{4} & \textbf{6.878} & \textbf{0.861} & \textbf{7.349} & \textbf{0.093} &\textbf{0.047} &\textbf{0.034} \\ 
\midrule
\multirow{48}{*}{20} & \multirow{16}{*}{10} & \multirow{8}{*}{Interacted distance} & \multirow{1}{*}{0.0001} & 3.553 & \underline{0.267} & 3.654 & 0.002 &\underline{0.626} &0.002 \\ 
& & &\multirow{1}{*}{0.001} & 3.548 & \underline{0.267} & 3.649 & 0.003 &\underline{0.626} &0.003 \\ 
& & &\multirow{1}{*}{0.01} & 3.552 & \underline{0.267} & 3.652 & 0.002 &\underline{0.626} &0.002 \\ 
& & &\multirow{1}{*}{0.1} & 3.558 & \textbf{0.268} & 3.659 & \underline{0.001} &\textbf{0.625} &\underline{0.0} \\ 
& & &\multirow{1}{*}{0.5} & \textbf{3.564} & \textbf{0.268} & \textbf{3.663} & \textbf{-0.001} &\textbf{0.625} &\textbf{-0.001} \\ 
& & &\multirow{1}{*}{1} & \underline{3.562} & \textbf{0.268} & \underline{3.662} & \textbf{-0.001} &\textbf{0.625} &\underline{-0.0} \\ 
& & &\multirow{1}{*}{2} & \underline{3.562} & \textbf{0.268} & \underline{3.662} & \textbf{-0.001} &\textbf{0.625} &\underline{-0.0} \\ 
& & &\multirow{1}{*}{4} & 3.55 & \underline{0.267} & 3.65 & 0.003 &\underline{0.626} &0.003 \\ 
\cmidrule{3-10}
& &\multirow{8}{*}{Coverage} & \multirow{1}{*}{0.0001} & 3.215 & 0.61 & 3.457 & 0.097 &0.146 &0.056 \\ 
& & &\multirow{1}{*}{0.001} & 3.219 & 0.611 & 3.461 & 0.096 &0.145 &0.054 \\ 
& & &\multirow{1}{*}{0.01} & 3.211 & 0.61 & 3.455 & 0.098 &0.146 &0.056 \\ 
& & &\multirow{1}{*}{0.1} & 3.218 & 0.611 & 3.46 & 0.096 &0.145 &0.055 \\ 
& & &\multirow{1}{*}{0.5} & 3.223 & \underline{0.613} & 3.466 & 0.095 &\underline{0.142} &0.053 \\ 
& & &\multirow{1}{*}{1} & 3.225 & \underline{0.613} & 3.469 & \underline{0.094} &\underline{0.142} &\underline{0.052} \\ 
& & &\multirow{1}{*}{2} & \textbf{3.23} & \textbf{0.614} & \underline{3.472} & \textbf{0.093} &\textbf{0.141} &\textbf{0.051} \\ 
& & &\multirow{1}{*}{4} & \underline{3.229} & \textbf{0.614} & \textbf{3.473} & \textbf{0.093} &\textbf{0.141} &\textbf{0.051} \\ 
\cmidrule{2-10}
& \multirow{16}{*}{20} & \multirow{8}{*}{Interacted distance} & \multirow{1}{*}{0.0001} & 5.233 & \textbf{0.385} & 5.285 & 0.002 &\textbf{0.534} &0.002 \\ 
& & &\multirow{1}{*}{0.001} & 5.234 & \underline{0.384} & 5.285 & 0.002 &\underline{0.535} &0.002 \\ 
& & &\multirow{1}{*}{0.01} & \textbf{5.241} & \textbf{0.385} & \textbf{5.292} & \textbf{0.0} &\textbf{0.534} &\textbf{0.0} \\ 
& & &\multirow{1}{*}{0.1} & 5.235 & \underline{0.384} & 5.286 & 0.002 &\underline{0.535} &\underline{0.001} \\ 
& & &\multirow{1}{*}{0.5} & 5.239 & \textbf{0.385} & \underline{5.291} & \underline{0.001} &\textbf{0.534} &\textbf{0.0} \\ 
& & &\multirow{1}{*}{1} & 5.23 & \underline{0.384} & 5.283 & 0.003 &\underline{0.535} &0.002 \\ 
& & &\multirow{1}{*}{2} & 5.238 & \textbf{0.385} & \underline{5.291} & \underline{0.001} &\textbf{0.534} &\textbf{0.0} \\ 
& & &\multirow{1}{*}{4} & \underline{5.24} & \textbf{0.385} & \textbf{5.292} & \underline{0.001} &\textbf{0.534} &\textbf{0.0} \\ 
\cmidrule{3-10}
& &\multirow{8}{*}{Coverage} & \multirow{1}{*}{0.0001} & 4.753 & 0.737 & 5.021 & 0.094 &0.108 &0.051 \\ 
& & &\multirow{1}{*}{0.001} & 4.743 & 0.736 & 5.01 & 0.095 &0.109 &0.054 \\ 
& & &\multirow{1}{*}{0.01} & 4.753 & 0.737 & 5.02 & 0.094 &0.108 &0.052 \\ 
& & &\multirow{1}{*}{0.1} & 4.737 & 0.736 & 5.004 & 0.097 &0.109 &0.055 \\ 
& & &\multirow{1}{*}{0.5} & 4.755 & 0.738 & 5.023 & 0.093 &0.107 &0.051 \\ 
& & &\multirow{1}{*}{1} & \underline{4.769} & \textbf{0.74} & \underline{5.036} & \underline{0.091} &\textbf{0.104} &\underline{0.049} \\ 
& & &\multirow{1}{*}{2} & 4.752 & \underline{0.739} & 5.019 & 0.094 &\underline{0.105} &0.052 \\ 
& & &\multirow{1}{*}{4} & \textbf{4.77} & \textbf{0.74} & \textbf{5.038} & \textbf{0.09} &\textbf{0.104} &\textbf{0.048} \\ 
\cmidrule{2-10}
& \multirow{16}{*}{40} & \multirow{8}{*}{Interacted distance} & \multirow{1}{*}{0.0001} & 7.521 & \underline{0.532} & 7.563 & 0.008 &\underline{0.411} &0.006 \\ 
& & &\multirow{1}{*}{0.001} & 7.523 & \underline{0.532} & 7.565 & 0.008 &\underline{0.411} &0.006 \\ 
& & &\multirow{1}{*}{0.01} & 7.53 & \underline{0.532} & 7.572 & \underline{0.007} &\underline{0.411} &\underline{0.005} \\ 
& & &\multirow{1}{*}{0.1} & 7.518 & 0.531 & 7.56 & 0.009 &0.412 &0.006 \\ 
& & &\multirow{1}{*}{0.5} & 7.517 & \underline{0.532} & 7.56 & 0.009 &\underline{0.411} &0.006 \\ 
& & &\multirow{1}{*}{1} & \textbf{7.539} & \textbf{0.533} & \textbf{7.582} & \textbf{0.006} &\textbf{0.41} &\textbf{0.004} \\ 
& & &\multirow{1}{*}{2} & 7.509 & 0.531 & 7.553 & 0.01 &0.412 &0.007 \\ 
& & &\multirow{1}{*}{4} & \underline{7.532} & \textbf{0.533} & \underline{7.577} & \underline{0.007} &\textbf{0.41} &\textbf{0.004} \\ 
\cmidrule{3-10}
& &\multirow{8}{*}{Coverage} & \multirow{1}{*}{0.0001} & 6.831 & 0.84 & 7.289 & 0.099 &0.07 &0.042 \\ 
& & &\multirow{1}{*}{0.001} & 6.832 & 0.84 & 7.289 & 0.099 &0.07 &0.042 \\ 
& & &\multirow{1}{*}{0.01} & 6.84 & 0.841 & 7.298 & 0.098 &0.069 &0.041 \\ 
& & &\multirow{1}{*}{0.1} & 6.852 & 0.841 & 7.313 & 0.097 &0.069 &\underline{0.039} \\ 
& & &\multirow{1}{*}{0.5} & \underline{6.856} & \underline{0.842} & \underline{7.314} & \underline{0.096} &\underline{0.068} &\underline{0.039} \\ 
& & &\multirow{1}{*}{1} & \textbf{6.867} & \textbf{0.843} & \textbf{7.328} & \textbf{0.095} &\textbf{0.067} &\textbf{0.037} \\ 
& & &\multirow{1}{*}{2} & 6.846 & \textbf{0.843} & 7.303 & 0.097 &\textbf{0.067} &0.04 \\ 
& & &\multirow{1}{*}{4} & 6.848 & \textbf{0.843} & 7.306 & 0.097 &\textbf{0.067} &0.04 \\ 

\end{tabular}}
\caption{Experiments over movielens-1m adopting jaccard distance in terms of genres. Results have been obtained by averaging 20 independent trails. Bold and underline values represent the best and second-best scores, respectively.}
\label{tab:jaccard_genres_movielens-1m_scores_table}
\end{table*}

==> movielens-1m/deterministic_jaccard_genres_scores_table.tex <==
\resizebox{\columnwidth}{!}{\begin{tabular}{c c c c c c c c c}
$k$ & $B$ & Strategy & \multicolumn{1}{c}{$D(C)$} & \multicolumn{1}{c}{$\textit{cov(C)}$} & \multicolumn{1}{c}{\textit{steps}} &\multicolumn{1}{c}{$\Delta_{\mathbbm{E[\textit{D}]}}$} & \multicolumn{1}{c}{$\Delta_{\mathbbm{E[\textit{cov}]}}$} &\multicolumn{1}{c}{$\Delta_{\mathbbm{E[\textit{steps}}]}$} \\ 
\midrule
\multirow{21}{*}{2} & \multirow{7}{*}{10} & \multirow{1}{*}{Relevance} & 2.65 & 0.19 & 3.66 & 0.26 &0.73 &0.0 \\ 
\cmidrule{3-9}
& &\multirow{1}{*}{Interacted distance} & \textbf{3.55} & 0.26 & 3.65 & \textbf{0.0} &0.64 &0.0 \\ 
& &\multirow{1}{*}{Coverage} & 3.31 & \textbf{0.69} & 3.51 & 0.07 &\textbf{0.03} &0.04 \\ 
\cmidrule{3-9}
& &\multirow{1}{*}{MMR} & 2.55 & 0.24 & 3.33 & 0.28 &0.66 &0.09 \\ 
& &\multirow{1}{*}{DUM} & 2.83 & 0.2 & 3.65 & 0.21 &0.72 &0.0 \\ 
& &\multirow{1}{*}{DPP} & 2.97 & 0.25 & 3.66 & 0.17 &0.65 &0.0 \\ 
& &\multirow{1}{*}{DGREC} & 2.43 & 0.23 & 3.07 & 0.32 &0.68 &0.16 \\ 
\cmidrule{2-9}
& \multirow{7}{*}{20} & \multirow{1}{*}{Relevance} & 3.89 & 0.24 & 5.28 & 0.26 &0.71 &0.0 \\ 
\cmidrule{3-9}
& &\multirow{1}{*}{Interacted distance} & \textbf{5.23} & 0.37 & 5.28 & \textbf{0.0} &0.55 &0.0 \\ 
& &\multirow{1}{*}{Coverage} & 4.89 & \textbf{0.8} & 5.13 & 0.07 &\textbf{0.03} &0.03 \\ 
\cmidrule{3-9}
& &\multirow{1}{*}{MMR} & 3.53 & 0.3 & 4.71 & 0.33 &0.64 &0.11 \\ 
& &\multirow{1}{*}{DUM} & 4.16 & 0.26 & 5.29 & 0.21 &0.69 &0.0 \\ 
& &\multirow{1}{*}{DPP} & 4.36 & 0.31 & 5.3 & 0.17 &0.62 &-0.0 \\ 
& &\multirow{1}{*}{DGREC} & 3.56 & 0.28 & 4.36 & 0.32 &0.66 &0.18 \\ 
\cmidrule{2-9}
& \multirow{7}{*}{40} & \multirow{1}{*}{Relevance} & 5.64 & 0.29 & 7.61 & 0.26 &0.68 &-0.0 \\ 
\cmidrule{3-9}
& &\multirow{1}{*}{Interacted distance} & \textbf{7.51} & 0.52 & 7.54 & \textbf{0.01} &0.42 &0.01 \\ 
& &\multirow{1}{*}{Coverage} & 6.95 & \textbf{0.89} & 7.44 & 0.08 &\textbf{0.01} &0.02 \\ 
\cmidrule{3-9}
& &\multirow{1}{*}{MMR} & 4.83 & 0.36 & 6.72 & 0.36 &0.6 &0.12 \\ 
& &\multirow{1}{*}{DUM} & 6.0 & 0.32 & 7.59 & 0.21 &0.65 &0.0 \\ 
& &\multirow{1}{*}{DPP} & 6.26 & 0.37 & 7.61 & 0.17 &0.59 &-0.0 \\ 
& &\multirow{1}{*}{DGREC} & 5.13 & 0.35 & 6.2 & 0.32 &0.61 &0.19 \\ 
\midrule
\multirow{21}{*}{10} & \multirow{7}{*}{10} & \multirow{1}{*}{Relevance} & 2.64 & 0.19 & 3.66 & 0.26 &0.73 &0.0 \\ 
\cmidrule{3-9}
& &\multirow{1}{*}{Interacted distance} & \textbf{3.56} & 0.26 & 3.66 & \textbf{0.0} &0.64 &0.0 \\ 
& &\multirow{1}{*}{Coverage} & 3.24 & \textbf{0.64} & 3.47 & 0.09 &\textbf{0.1} &0.05 \\ 
\cmidrule{3-9}
& &\multirow{1}{*}{MMR} & 3.02 & 0.24 & 3.47 & 0.15 &0.66 &0.05 \\ 
& &\multirow{1}{*}{DUM} & 3.18 & 0.27 & 3.65 & 0.11 &0.62 &0.0 \\ 
& &\multirow{1}{*}{DPP} & 3.33 & 0.24 & 3.66 & 0.06 &0.66 &0.0 \\ 
& &\multirow{1}{*}{DGREC} & 2.25 & 0.21 & 2.9 & 0.37 &0.71 &0.21 \\ 
\cmidrule{2-9}
& \multirow{7}{*}{20} & \multirow{1}{*}{Relevance} & 3.91 & 0.24 & 5.3 & 0.25 &0.71 &-0.0 \\ 
\cmidrule{3-9}
& &\multirow{1}{*}{Interacted distance} & \textbf{5.24} & 0.38 & 5.29 & \textbf{0.0} &0.54 &0.0 \\ 
& &\multirow{1}{*}{Coverage} & 4.78 & \textbf{0.76} & 5.04 & 0.09 &\textbf{0.08} &0.05 \\ 
\cmidrule{3-9}
& &\multirow{1}{*}{MMR} & 4.25 & 0.31 & 4.88 & 0.19 &0.62 &0.08 \\ 
& &\multirow{1}{*}{DUM} & 4.7 & 0.36 & 5.3 & 0.1 &0.56 &-0.0 \\ 
& &\multirow{1}{*}{DPP} & 4.9 & 0.33 & 5.3 & 0.07 &0.6 &-0.0 \\ 
& &\multirow{1}{*}{DGREC} & 3.27 & 0.27 & 4.05 & 0.38 &0.67 &0.23 \\ 
\cmidrule{2-9}
& \multirow{7}{*}{40} & \multirow{1}{*}{Relevance} & 5.65 & 0.29 & \textbf{7.6} & 0.26 &0.68 &\textbf{0.0} \\ 
\cmidrule{3-9}
& &\multirow{1}{*}{Interacted distance} & \textbf{7.51} & 0.52 & 7.55 & \textbf{0.01} &0.42 &0.01 \\ 
& &\multirow{1}{*}{Coverage} & 6.85 & \textbf{0.86} & 7.32 & 0.1 &\textbf{0.05} &0.04 \\ 
\cmidrule{3-9}
& &\multirow{1}{*}{MMR} & 5.85 & 0.38 & 6.81 & 0.23 &0.58 &0.11 \\ 
& &\multirow{1}{*}{DUM} & 6.78 & 0.45 & \textbf{7.6} & 0.11 &0.5 &\textbf{0.0} \\ 
& &\multirow{1}{*}{DPP} & 7.07 & 0.43 & \textbf{7.6} & 0.07 &0.52 &\textbf{0.0} \\ 
& &\multirow{1}{*}{DGREC} & 4.64 & 0.33 & 5.65 & 0.39 &0.63 &0.26 \\ 
\midrule
\multirow{21}{*}{20} & \multirow{7}{*}{10} & \multirow{1}{*}{Relevance} & 2.64 & 0.19 & 3.65 & 0.26 &0.73 &0.0 \\ 
\cmidrule{3-9}
& &\multirow{1}{*}{Interacted distance} & \textbf{3.56} & 0.27 & 3.66 & \textbf{0.0} &0.62 &0.0 \\ 
& &\multirow{1}{*}{Coverage} & 3.22 & \textbf{0.61} & 3.47 & 0.1 &\textbf{0.15} &0.05 \\ 
\cmidrule{3-9}
& &\multirow{1}{*}{MMR} & 3.01 & 0.27 & 3.51 & 0.15 &0.62 &0.04 \\ 
& &\multirow{1}{*}{DUM} & 3.19 & 0.3 & 3.66 & 0.1 &0.58 &0.0 \\ 
& &\multirow{1}{*}{DPP} & 3.33 & 0.29 & 3.67 & 0.06 &0.59 &-0.0 \\ 
& &\multirow{1}{*}{DGREC} & 2.26 & 0.21 & 2.91 & 0.37 &0.71 &0.2 \\ 
\cmidrule{2-9}
& \multirow{7}{*}{20} & \multirow{1}{*}{Relevance} & 3.9 & 0.24 & 5.29 & 0.26 &0.71 &0.0 \\ 
\cmidrule{3-9}
& &\multirow{1}{*}{Interacted distance} & \textbf{5.24} & 0.38 & 5.29 & \textbf{0.0} &0.54 &0.0 \\ 
& &\multirow{1}{*}{Coverage} & 4.76 & \textbf{0.74} & 5.02 & 0.09 &\textbf{0.1} &0.05 \\ 
\cmidrule{3-9}
& &\multirow{1}{*}{MMR} & 4.28 & 0.33 & 4.96 & 0.18 &0.6 &0.06 \\ 
& &\multirow{1}{*}{DUM} & 4.7 & 0.39 & 5.29 & 0.1 &0.53 &0.0 \\ 
& &\multirow{1}{*}{DPP} & 4.9 & 0.38 & 5.3 & 0.07 &0.54 &-0.0 \\ 
& &\multirow{1}{*}{DGREC} & 3.32 & 0.27 & 4.11 & 0.37 &0.67 &0.22 \\ 
\cmidrule{2-9}
& \multirow{7}{*}{40} & \multirow{1}{*}{Relevance} & 5.65 & 0.29 & 7.6 & 0.26 &0.68 &0.0 \\ 
\cmidrule{3-9}
& &\multirow{1}{*}{Interacted distance} & \textbf{7.52} & 0.53 & 7.56 & \textbf{0.01} &0.41 &0.01 \\ 
& &\multirow{1}{*}{Coverage} & 6.86 & \textbf{0.84} & 7.31 & 0.1 &\textbf{0.07} &0.04 \\ 
\cmidrule{3-9}
& &\multirow{1}{*}{MMR} & 5.96 & 0.4 & 6.96 & 0.21 &0.56 &0.09 \\ 
& &\multirow{1}{*}{DUM} & 6.79 & 0.48 & 7.6 & 0.1 &0.47 &0.0 \\ 
& &\multirow{1}{*}{DPP} & 7.09 & 0.48 & 7.62 & 0.07 &0.47 &-0.0 \\ 
& &\multirow{1}{*}{DGREC} & 4.74 & 0.34 & 5.78 & 0.38 &0.62 &0.24 \\ 
\midrule
\end{tabular}}
\caption{Results on Movielens-1M. The best scores with a statistical significance $p<0.05$ are highlighted in bold.}
\label{tab:jaccard_genres_movielens-1m_scores_table}
 

==> movielens-1m/partial_scores_table.tex <==
\begin{table*}
 \centering 
\resizebox{0.6\textwidth}{!}{\begin{tabular}{c|c|c|c|c|c|c|c|c}
\hline 
Dataset & Patience & Rec Strategy & \multicolumn{1}{c|}{R(C)} & \multicolumn{1}{c|}{cov(C)} & \multicolumn{1}{c|}{steps} &\multicolumn{1}{c|}{$\delta_R$} & \multicolumn{1}{c|}{$\delta_{cov}$} &\multicolumn{1}{c}{$\delta_{steps}$} \\ 
\hline\hline
\multirow{21}{*}{\rotatebox{90}{Movielens-1M}} & \multirow{7}{*}{10} & \multirow{1}{*}{relevance} & 9.51 & 0.19 & \textbf{3.66} & -1.67 &0.73 &\textbf{0.0} \\ 
\cline{3-9}
& &\multirow{1}{*}{interacted distance w relevance} & \textbf{12.62} & 0.26 & \underline{3.65} & \textbf{-2.54} &0.64 &\textbf{0.0} \\ 
& &\multirow{1}{*}{coverage w relevance} & 10.96 & \textbf{0.64} & 3.47 & -2.08 &\textbf{0.1} &\underline{0.05} \\ 
\cline{3-9}
& &\multirow{1}{*}{mmr} & 9.93 & 0.24 & 3.47 & -1.79 &0.66 &\underline{0.05} \\ 
& &\multirow{1}{*}{dpp} & \underline{11.79} & 0.24 & \textbf{3.66} & \underline{-2.31} &0.66 &\textbf{0.0} \\ 
& &\multirow{1}{*}{dum} & 11.38 & \underline{0.27} & \textbf{3.66} & -2.2 &\underline{0.62} &\textbf{0.0} \\ 
& &\multirow{1}{*}{dgrec} & 6.28 & 0.21 & 2.89 & -0.76 &0.71 &0.21 \\ 
\hhline{~========}
& \multirow{7}{*}{20} & \multirow{1}{*}{relevance} & 22.04 & 0.24 & \underline{5.29} & -3.2 &0.71 &\textbf{0.0} \\ 
\cline{3-9}
& &\multirow{1}{*}{interacted distance w relevance} & \textbf{29.12} & \underline{0.38} & 5.27 & \textbf{-4.55} &\underline{0.54} &\textbf{0.0} \\ 
& &\multirow{1}{*}{coverage w relevance} & 25.6 & \textbf{0.76} & 5.03 & -3.88 &\textbf{0.08} &\underline{0.05} \\ 
\cline{3-9}
& &\multirow{1}{*}{mmr} & 21.1 & 0.31 & 4.85 & -3.02 &0.62 &0.08 \\ 
& &\multirow{1}{*}{dpp} & \underline{27.52} & 0.33 & \textbf{5.3} & \underline{-4.25} &0.6 &\textbf{-0.0} \\ 
& &\multirow{1}{*}{dum} & 26.31 & 0.35 & \underline{5.29} & -4.02 &0.58 &\textbf{0.0} \\ 
& &\multirow{1}{*}{dgrec} & 13.92 & 0.27 & 4.06 & -1.65 &0.67 &0.23 \\ 
\hhline{~========}
& \multirow{7}{*}{40} & \multirow{1}{*}{relevance} & 48.62 & 0.29 & \underline{7.61} & -5.41 &0.68 &\textbf{0.0} \\ 
\cline{3-9}
& &\multirow{1}{*}{interacted distance w relevance} & \textbf{63.21} & \underline{0.52} & 7.54 & \textbf{-7.33} &\underline{0.42} &\underline{0.01} \\ 
& &\multirow{1}{*}{coverage w relevance} & 56.36 & \textbf{0.86} & 7.31 & -6.43 &\textbf{0.05} &0.04 \\ 
\cline{3-9}
& &\multirow{1}{*}{mmr} & 43.0 & 0.38 & 6.78 & -4.67 &0.58 &0.11 \\ 
& &\multirow{1}{*}{dpp} & \underline{60.56} & 0.42 & \textbf{7.62} & \underline{-6.99} &0.53 &\textbf{-0.0} \\ 
& &\multirow{1}{*}{dum} & 57.69 & 0.44 & 7.59 & -6.61 &0.51 &\textbf{0.0} \\ 
& &\multirow{1}{*}{dgrec} & 29.15 & 0.33 & 5.67 & -2.84 &0.63 &0.25 \\ 
\hline
\end{tabular}}
%\caption{Experiments over movielens-1m adopting jaccard distance in terms of genres. Results have been obtained by averaging 20 independent trails. Bold and underline values represent the best and second-best scores, respectively.}
\label{tab:jaccard_genres_movielens-1m_scores_table}
\end{table*}

==> netflix/deterministic_jaccard_genres_scores_table.tex <==
\resizebox{\textwidth}{!}{\begin{tabular}{c c c c c c c c c}
$k$ & $B$ & Strategy & \multicolumn{1}{c}{$D(C)$} & \multicolumn{1}{c}{$\textit{cov(C)}$} & \multicolumn{1}{c}{\textit{steps}} &\multicolumn{1}{c}{$\Delta_{\mathbbm{E[\textit{D}]}}$} & \multicolumn{1}{c}{$\Delta_{\mathbbm{E[\textit{cov}]}}$} &\multicolumn{1}{c}{$\Delta_{\mathbbm{E[\textit{steps}}]}$} \\
\midrule
\multirow{21}{*}{2} & \multirow{7}{*}{10} & \multirow{1}{*}{Relevance} & 2.94 & 0.27 & 3.58 & 0.17 &0.62 &0.02 \\ 
\cmidrule{3-9}
& &\multirow{1}{*}{Interacted distance} & \textbf{3.43} & 0.3 & 3.54 & \textbf{0.04} &0.58 &0.03 \\ 
& &\multirow{1}{*}{Coverage} & 3.01 & \textbf{0.59} & 3.4 & 0.15 &\textbf{0.17} &0.07 \\ 
\cmidrule{3-9}
& &\multirow{1}{*}{MMR} & 2.67 & 0.26 & 3.24 & 0.25 &0.63 &0.11 \\ 
& &\multirow{1}{*}{DUM} & 2.95 & 0.28 & 3.58 & 0.17 &0.61 &0.02 \\ 
& &\multirow{1}{*}{DPP} & 3.06 & 0.28 & 3.59 & 0.14 &0.61 &0.02 \\ 
& &\multirow{1}{*}{DGREC} & 2.5 & 0.25 & 3.14 & 0.3 &0.65 &0.14 \\ 
\cmidrule{2-9}
& \multirow{7}{*}{20} & \multirow{1}{*}{Relevance} & 4.32 & 0.34 & 5.16 & 0.18 &0.57 &0.03 \\ 
\cmidrule{3-9}
& &\multirow{1}{*}{Interacted distance} & \textbf{4.99} & 0.4 & 5.06 & \textbf{0.05} &0.49 &0.04 \\ 
& &\multirow{1}{*}{Coverage} & 4.43 & \textbf{0.69} & 4.86 & 0.16 &\textbf{0.12} &0.08 \\ 
\cmidrule{3-9}
& &\multirow{1}{*}{MMR} & 3.83 & 0.33 & 4.59 & 0.27 &0.58 &0.13 \\ 
& &\multirow{1}{*}{DUM} & 4.34 & 0.34 & 5.17 & 0.17 &0.57 &0.02 \\ 
& &\multirow{1}{*}{DPP} & 4.47 & 0.35 & 5.16 & 0.15 &0.56 &0.03 \\ 
& &\multirow{1}{*}{DGREC} & 2.92 & 0.24 & 4.76 & 0.44 &0.7 &0.1 \\ 
\cmidrule{2-9}
& \multirow{7}{*}{40} & \multirow{1}{*}{Relevance} & 6.22 & 0.41 & 7.39 & 0.18 &0.52 &0.03 \\ 
\cmidrule{3-9}
& &\multirow{1}{*}{Interacted distance} & \textbf{7.07} & 0.52 & 7.16 & \textbf{0.07} &0.39 &0.06 \\ 
& &\multirow{1}{*}{Coverage} & 6.39 & \textbf{0.77} & 6.93 & 0.16 &\textbf{0.09} &0.09 \\ 
\cmidrule{3-9}
& &\multirow{1}{*}{MMR} & 5.37 & 0.39 & 6.5 & 0.29 &0.54 &0.15 \\ 
& &\multirow{1}{*}{DUM} & 6.21 & 0.41 & 7.36 & 0.18 &0.52 &0.03 \\ 
& &\multirow{1}{*}{DPP} & 6.4 & 0.42 & 7.38 & 0.16 &0.5 &0.03 \\ 
& &\multirow{1}{*}{DGREC} & 4.28 & 0.28 & 6.77 & 0.44 &0.67 &0.11 \\ 
\midrule
\multirow{21}{*}{10} & \multirow{7}{*}{10} & \multirow{1}{*}{Relevance} & 2.95 & 0.27 & \textbf{3.59} & 0.17 &0.62 &\textbf{0.02} \\ 
\cmidrule{3-9}
& &\multirow{1}{*}{Interacted distance} & \textbf{3.42} & 0.3 & 3.55 & \textbf{0.04} &0.58 &0.03 \\ 
& &\multirow{1}{*}{Coverage} & 2.94 & \textbf{0.54} & 3.36 & 0.17 &\textbf{0.24} &0.08 \\ 
\cmidrule{3-9}
& &\multirow{1}{*}{MMR} & 2.72 & 0.26 & 3.23 & 0.24 &0.63 &0.12 \\ 
& &\multirow{1}{*}{DUM} & 3.01 & 0.31 & \textbf{3.59} & 0.15 &0.56 &\textbf{0.02} \\ 
& &\multirow{1}{*}{DPP} & 3.18 & 0.28 & \textbf{3.59} & 0.11 &0.61 &\textbf{0.02} \\ 
& &\multirow{1}{*}{DGREC} & 2.05 & 0.22 & 3.26 & 0.42 &0.69 &0.11 \\ 
\cmidrule{2-9}
& \multirow{7}{*}{20} & \multirow{1}{*}{Relevance} & 4.34 & 0.34 & 5.19 & 0.17 &0.57 &0.02 \\ 
\cmidrule{3-9}
& &\multirow{1}{*}{Interacted distance} & \textbf{4.97} & 0.4 & 5.07 & \textbf{0.05} &0.49 &0.04 \\ 
& &\multirow{1}{*}{Coverage} & 4.33 & \textbf{0.64} & 4.79 & 0.17 &\textbf{0.19} &0.1 \\ 
\cmidrule{3-9}
& &\multirow{1}{*}{MMR} & 3.86 & 0.32 & 4.51 & 0.26 &0.59 &0.15 \\ 
& &\multirow{1}{*}{DUM} & 4.44 & 0.38 & 5.2 & 0.15 &0.52 &0.02 \\ 
& &\multirow{1}{*}{DPP} & 4.68 & 0.36 & 5.19 & 0.11 &0.54 &0.02 \\ 
& &\multirow{1}{*}{DGREC} & 3.01 & 0.26 & 4.63 & 0.43 &0.67 &0.13 \\ 
\cmidrule{2-9}
& \multirow{7}{*}{40} & \multirow{1}{*}{Relevance} & 6.24 & 0.41 & 7.42 & 0.18 &0.52 &0.02 \\ 
\cmidrule{3-9}
& &\multirow{1}{*}{Interacted distance} & \textbf{7.03} & 0.51 & 7.16 & \textbf{0.07} &0.4 &0.06 \\ 
& &\multirow{1}{*}{Coverage} & 6.18 & \textbf{0.73} & 6.77 & 0.19 &\textbf{0.14} &0.11 \\ 
\cmidrule{3-9}
& &\multirow{1}{*}{MMR} & 5.38 & 0.39 & 6.29 & 0.29 &0.54 &0.17 \\ 
& &\multirow{1}{*}{DUM} & 6.4 & 0.46 & 7.45 & 0.16 &0.46 &0.02 \\ 
& &\multirow{1}{*}{DPP} & 6.73 & 0.44 & 7.42 & 0.11 &0.48 &0.02 \\ 
& &\multirow{1}{*}{DGREC} & 4.38 & 0.3 & 6.6 & 0.42 &0.65 &0.13 \\ 
\midrule
\multirow{21}{*}{20} & \multirow{7}{*}{10} & \multirow{1}{*}{Relevance} & 2.95 & 0.27 & 3.61 & 0.17 &0.62 &0.01 \\ 
\cmidrule{3-9}
& &\multirow{1}{*}{Interacted distance} & \textbf{3.41} & 0.31 & 3.55 & \textbf{0.04} &0.56 &0.03 \\ 
& &\multirow{1}{*}{Coverage} & 2.93 & \textbf{0.52} & 3.35 & 0.18 &\textbf{0.27} &0.08 \\ 
\cmidrule{3-9}
& &\multirow{1}{*}{MMR} & 2.7 & 0.26 & 3.23 & 0.24 &0.63 &0.12 \\ 
& &\multirow{1}{*}{DUM} & 3.09 & 0.3 & 3.59 & 0.13 &0.58 &0.02 \\ 
& &\multirow{1}{*}{DPP} & 3.21 & 0.28 & 3.61 & 0.1 &0.61 &0.01 \\ 
& &\multirow{1}{*}{DGREC} & 2.17 & 0.22 & 3.27 & 0.39 &0.69 &0.11 \\ 
\cmidrule{2-9}
& \multirow{7}{*}{20} & \multirow{1}{*}{Relevance} & 4.33 & 0.34 & \textbf{5.2} & 0.17 &0.57 &\textbf{0.02} \\ 
\cmidrule{3-9}
& &\multirow{1}{*}{Interacted distance} & \textbf{4.98} & 0.41 & 5.11 & \textbf{0.05} &0.48 &0.03 \\ 
& &\multirow{1}{*}{Coverage} & 4.33 & \textbf{0.62} & 4.81 & 0.17 &\textbf{0.21} &0.09 \\ 
\cmidrule{3-9}
& &\multirow{1}{*}{MMR} & 3.86 & 0.32 & 4.54 & 0.26 &0.59 &0.14 \\ 
& &\multirow{1}{*}{DUM} & 4.56 & 0.38 & \textbf{5.2} & 0.13 &0.52 &\textbf{0.02} \\ 
& &\multirow{1}{*}{DPP} & 4.71 & 0.36 & \textbf{5.2} & 0.1 &0.54 &\textbf{0.02} \\ 
& &\multirow{1}{*}{DGREC} & 3.2 & 0.27 & 4.67 & 0.39 &0.66 &0.12 \\ 
\cmidrule{2-9}
& \multirow{7}{*}{40} & \multirow{1}{*}{Relevance} & 6.23 & 0.41 & 7.44 & 0.18 &0.52 &0.02 \\ 
\cmidrule{3-9}
& &\multirow{1}{*}{Interacted distance} & \textbf{7.01} & 0.51 & 7.19 & \textbf{0.08} &0.4 &0.06 \\ 
& &\multirow{1}{*}{Coverage} & 6.18 & \textbf{0.71} & 6.8 & 0.19 &\textbf{0.16} &0.11 \\ 
\cmidrule{3-9}
& &\multirow{1}{*}{MMR} & 5.4 & 0.39 & 6.35 & 0.29 &0.54 &0.17 \\ 
& &\multirow{1}{*}{DUM} & 6.57 & 0.47 & 7.46 & 0.13 &0.44 &0.02 \\ 
& &\multirow{1}{*}{DPP} & 6.8 & 0.45 & 7.45 & 0.1 &0.47 &0.02 \\ 
& &\multirow{1}{*}{DGREC} & 4.6 & 0.31 & 6.63 & 0.39 &0.63 &0.13 \\ 
\midrule
\end{tabular}}
\caption{Results on Netflix. The best scores with a statistical significance $p<0.05$ are highlighted in bold.}
\label{tab:weibull_netflix_scores}
 

==> webconf_abstract.tex <==
\iffalse
    \textit{Diversity} has been fully-fledged recognized as a significant factor in evaluating the quality of a recommendation algorithm, since it is proven to both increase user satisfaction and play a central role in alleviating detrimental effects on online platforms, such as \textit{filter bubble}, \textit{echo chambers} and \textit{fake news spread}.
    For this reason, in this work, we tackle the problem of diversity from an innovative perspective. First of all, we define two measures to quantify the diversity induced by a recommendation algorithm, either at item- or group-level. Second, we propose a  simulation methodology that is user-aware, i.e., allows users to \textit{stop} interacting with the algorithm if the recommendations are not relevant. In this way, we prove to induce a strong interplay between \textit{relevance}, \textit{diversity}, and \textit{user behavior}. Finally, we implement two novel recommendation strategies that account for both items' utility and diversity, by exploiting copula functions. To the best of our knowledge, this is the first attempt to adopt copulas in this context.
    We conduct an extensive evaluation of the proposed methodology over different benchmark datasets, and we show that our strategies overcome several state-of-the-art competitors.
\fi

%TLDR: We propose a new framework for designing recommender systems that cope with the trade-off of relevance vs. diversity. In the proposed framework, we model the users' response to recommendations, and we account for the fact that users will keep interacting with the system as long as they receive relevant recommendations. We propose maximizing diversity as a sole objective, but relevance is a necessary condition to achieve the diversity-maximization goal.

%\erica{Maybe we should change the word "exploration" with something conceptually similar. I was looking around for similar works, but the keyword "exploration" is always related with RL/Multi Armed Bandits. So I do not know if it is a good idea to adopt exactly this term. Maybe we can replace it with "discovery" or something like that.}

% \aris{OK, but discovery conveys a different idea than exploration. Can we use exploration and clarify that it does not fit under reinforcement learning? Btw, are there any recommender systems papers using reinforcement learning approaches? }

% \aris{I think that we should also say explicitly that our framework is designed for this type of information-exploration situations. There may be other situations, different than information exploration,  where a different kind of framework should be preferred. }

% \erica{Maybe we should insert a notation table?}

Providing recommendations that are \emph{relevant} as well as \emph{diverse} is a key consideration of modern recommendation systems for Web applications.
Optimizing both of these measures presents a fundamental trade-off, 
as increasing diversity typically comes at the cost of lower relevance, thus impairing the overall user engagement. 
Existing recommendation algorithms try to resolve this trade-off
by combining the two measures, relevance and diversity, into one objective
and then seeking recommendations that optimize the combined objective
while fixing the number of items to be recommended. 
Traditional approaches, however, do not consider
whether the user interacts with the recommended items or not.

In this paper, we put the \emph{user behavior} at the driver's seat of the performance of a recommendation system, by building on the interplay between \emph{relevance}, \emph{diversity}, and \emph{user behavior}.
More concretely, we view diversity as a surrogate of the total amount of knowledge obtained by the user while interacting with the system, 
and we seek to optimize diversity. We propose a probabilistic user-behavior model in which users keep interacting with the recommendation system
as long as they receive relevant recommendations, 
but they may stop if the relevance of the recommended items drops.
Thus, for a recommendation system to achieve a high-diversity measure in our model, it will need to produce recommendations that are \emph{both relevant and~diverse}.

Finally, we propose a novel recommendation strategy 
that combines relevance and diversity by a copula function. 
We conduct an extensive evaluation of the proposed methodology over different benchmark datasets, 
and we show that our strategy outperforms several state-of-the-art competitors.

The code for the experiments is accessible at the following url: \url{https://anonymous.4open.science/r/EXPLORE-AA84/}.


==> webconf_intro.tex <==
\section{Introduction}
\label{sec:introduction}

The widespread adoption of web-based services enables a growing number of users to access and engage with online content. Users visit web pages, make purchases on e-commerce websites, stream online content, and participate in social-networking platforms. Recommender systems play a central role in such applications, by helping users navigate Web catalogs, suggesting news articles~\cite{Wu2019NPANN}, music~\cite{Chen2018WSDMC2}, or advertisement~\cite{Gao2021LearningAE,Gu2020HierarchicalUP}.
Despite initially focusing on predicting users' interests and maximizing \emph{relevance}, \erica{as reported by Castells et al.~\cite{Castells2022},  the importance of diversity has been early recognized~\cite{evaluating_CF, Smyth2001SimilarityVD} as an added value for recommendations~\cite{first_diversification}. This awareness grew progressively, yielding to several improvements in the last decade~\cite{on_unexpectedness, improving_aggregate, evaluating_novel_recs, diversity_top_n_recs, rank_relevance}. Also, several online and targeted user studies assessed the increase in user satisfaction when diversity is incorporated into the list of suggested items~\cite{diversity_top_n_recs, Castells2022}. For example, Allison et al.~\cite{algorithmic_confounding} show that, if certain objectives (including diversity) are not taken into account, the interactions between users and recommender systems are prone to homogenization and, consequently, low utility. }
%\emph{diversity} is now recognized as an important aspect of recommender systems~\cite{first_diversification}.
\iffalse
Despite evaluating their quality was firstly reduced in estimating their capability in predicting users' interest, a wider perspective started to appear in the literature by the beginning of the 2000s~\cite{evaluating_CF, Smyth2001SimilarityVD}, when the property of \emph{diversity} started to be recognized in the added value of recommendations~\cite{first_diversification}.
\fi
Indeed, 
% beyond improving user satisfaction~\cite{explain, serendipity},
providing diverse recommendations can be critical in mitigating detrimental consequences,
%  due to excessive personalization on online platforms, 
% \textit{echo chambers} and \textit{filter bubbles}~\cite{Pariser2012TheFB}, 
such as being trapped in \emph{rabbit holes}\footnote{\erica{With the term \textit{rabbit holes}, we do not refer necessarily to the phenomenon of radicalization in a political context, but to a broader concept, in which the algorithm leads the user to consume limited types of content. 
%On the other hand, radicalization can be a topic related to diversity as well, since users could become exposed to partial information within a narrow community, which leads their beliefs and experiences to the extremes.
}} in platforms like Youtube~\cite{rabbit_hole, the_great_radicalizer, ribeiro2020auditing, Haroon2022YouTubeTG} or Reddit~\cite{phadke2022pathways}, 
where users can fall into conspiracy discussions~\cite{phadke2022pathways}
or promote the spread of misinformation~\cite{echo_chamber_fake_news, Trnberg2018EchoCA, spreading}.
% or follow polarized communities~\cite{Jiang2021SocialMP}.

In order to balance \emph{relevance} and \emph{diversity}, 
common approaches % for existing recommendation systems 
seek to combine the two measures
into one objective, and then optimize the combined objective.
%  for a given number of recommendations. 
Such approaches, however, do not take into account the \emph{user behavior} 
and the interaction of the users with the list of recommended items.

In this paper, we propose a new framework for designing recommender systems,
where we seek to balance \emph{relevance} and \emph{diversity}
guided by a \emph{user-behavior model}.
Our idea is to view the interaction of a user with an online platform as an \emph{exploration task}, 
and to view recommendations as a mechanism for enabling exploration. 
The objective is to maximize the amount of useful not-repetitive knowledge that 
a user accrues during exploration. 
We model the total amount of knowledge accrued by the user using a diversity measure, 
and consequently, we aim to maximize diversity. 
Although diversity is the sole objective in the optimization problem we define, 
the coupling of the exploration task with the user-behavior model 
implies that for a recommendation system to achieve high diversity
it will need to produce recommendations that are \emph{both relevant and~diverse}.
We illustrate the proposed concept of \emph{``information exploration via recommendations''} with the following example.

\begin{figure}
\centering
\begin{subfigure}[b]{0.3\columnwidth}
        \centering
        \includegraphics[width=0.25\columnwidth]{fig/diversity scenarios/scenario_1.png}
    \caption{}
    \end{subfigure}
    %
    \begin{subfigure}[b]{0.32\columnwidth}
        \centering
        \includegraphics[width=\columnwidth]{fig/diversity scenarios/scenario_2.png}
    \caption{}
    \end{subfigure}
    %
    \begin{subfigure}[b]{0.32\columnwidth}
        \centering
        \includegraphics[width=0.7\columnwidth]{fig/diversity scenarios/scenario_3.png}
    \caption{}
    \end{subfigure}
\caption{
\iffalse
Illustration of the effect of different recommendation strategies.
The white points represent recommended items, while the blue circles represent their ``information coverage'', e.g., the topics they are related to. 
The underlying space represents semantic distances between recommended items.
(a) Highly relevant recommendations keep the user engaged but they are too similar to each other, so the overall diversity is low (e.g., they are all about ``technology'').
(b) Highly diverse recommendations (e.g., covering ``technology,'' ``art,'' and ``lifestyle'') are likely to be non-relevant, and the user will lose interest after a small number of recommendations.
(c) A desirable trade-off between relevance and diversity; the recommendations are sufficiently relevant and diverse for the user to stay engaged 
and consume a diverse information diet (e.g., covering ``technology,'' ``science,'' and~``gaming'').
\fi
\erica{Illustration of recommendation strategies' impact. White points are recommended items, blue circles indicate "information coverage." (a) High relevance, low diversity (e.g., all about "technology"). (b) High diversity, likely non-relevant (e.g., "technology," "art," "lifestyle"). (c) Optimal balance: Relevant and diverse, keeping user engaged with varied topics like "technology," "science," "gaming."}
}
% \caption{Illustration of the effect of different recommendation strategies.
% The white points represent recommended items.
% The blue circle represent the ``information content'' of recommended items.
% \giuseppe{We should clarify what "information content" means cause it's a bit ambiguous. Maybe we can use "Information coverage", to denote the span that it covers (and hence the possible overlaps that allow propagation of relevance). Possible rewriting:  The blue circle represent the ``information coverage'' of recommended items like, e.g., the topics they are related to. }
% The underlying space (here 2-$d$) represents semantic distances between recommended items.
% (a) Highly relevant recommendations can keep the user engaged but
% the recommendations are likely too similar to each other, and the overall diversity is low\giuseppe{, e.g. cause they are all about "technology"}.
% (b) Highly diverse recommendations \giuseppe{(e.g., covering technology, arts and lifestyle)} are likely to be non relevant,
% and the user will loose interest after a small number of recommendations.
% (c) A desirable trade-off between relevance and diversity; 
% the recommendations are sufficiently relevant and diverse for the user to stay engaged 
% and consume a diverse information~diet.
% \aris{these are all great suggestions! Let's implement them.}
% }
\label{fig:diversity_scenarios}
\end{figure}

%\iffalse
\spara{Example.}
Consider a user, Alice, browsing a personalized Web application for finding 
interesting news articles to read.
The exploration process is iterative, and is depicted in Figure~\ref{fig:toy_example}. 
At each step, the Web application recommends a set of news articles to Alice, 
and Alice clicks on one of the articles to read. 
At some point, Alice decides to quit the Web application, 
either because she received enough information, 
or because the recommendations are not very interesting to her, 
or simply because she got bored.
Our goal is to design a recommendation algorithm that maximizes Alice's experience. While common approaches focus on maximizing engagement and time spent, we propose prioritizing the total information received by emphasizing diverse news articles. The challenge is to strike a balance between diversity and relevance to keep Alice engaged while exploring relevant and interesting topics, avoiding scenarios where recommendations are either too focused (Figure~\ref{fig:diversity_scenarios}(a)) or too diverse and irrelevant (Figure~\ref{fig:diversity_scenarios}(b)). Our aim is to create an ideal scenario (Figure~\ref{fig:diversity_scenarios}(c)) where Alice explores many relevant and interesting topics, enriching her knowledge.

\iffalse
Our question is,  
\emph{how should a recommendation algorithm be designed in order to maximize the experience of Alice?}
One approach, typically followed, 
is to maximize the engagement of Alice and the time spent on the application. 
This could be useful, for instance, for monetization purposes. 
Maximizing engagement, however, entails the risk of favoring a ``rabbit hole'' strategy, 
where the emphasis is to provide only highly relevant but not diverse recommendations for Alice.
The effect of such as strategy is illustrated in Figure~\ref{fig:diversity_scenarios}(a).

Instead, in this paper, we aim to maximize the total amount of information received by Alice. 
The intuition is to nudge Alice into receiving a well-rounded and informative news diet.
A meaningful way to achieve this is by aiming to maximize the diversity of news articles recommended,
and eventually read, by Alice.
However, in the prospect of Alice quitting the application if she receives recommendations that are not interesting to her, 
we need to ensure that \emph{recommendations are diverse yet relevant enough to keep her sufficiently engaged}. 
In a scenario of diverse but not relevant recommendations, illustrated in Figure~\ref{fig:diversity_scenarios}(b), 
Alice will lose interest quickly.
The ideal scenario, illustrated in Figure~\ref{fig:diversity_scenarios}(c), 
which defines our research challenge, 
is to find the right balance between diversity and relevance for Alice to explore 
many relevant and interesting topics and to enrich her knowledge.
\hfill$\Box$
\fi

% Moreover, the lack of diversity in information can lead to detrimental consequences by promoting the spread of misinformation~\cite{echo_chamber_fake_news, Trnberg2018EchoCA, spreading}: on Twitter and Facebook, the polarized communities were proven to be the main source of fake news proliferation related to the COVID-19 pandemic~\cite{Jiang2021SocialMP}, the 2016 US presidential election~\cite{us_election}, and the recent Russia-Ukrain war~\cite{russia_ukrain_war}.  

\iffalse
This given, reaching a good trade-off between personalization and a healthy degree of diversity is certainly crucial when designing online applications that rely on recommendation algorithms, so as to tackle the aforesaid noxious effects~\cite{Castells2022}. 

We address the discussed challenge by looking at the diversity problem from innovative perspectives. First of all, we model items' diversity as a \textit{total} and \textit{normalized} measure, i.e., we are interested in estimating ($i$) at which extent final user interactions are different from each other, and ($ii$) what is their average degree of diversity. In other words, we define a distance metric that does not quadratically grow with respect to the number of interactions but represents an average measure of distance among items, linear in their growth.  
Secondly, we develop a novel simulation framework that mimics user-recommender multiple interactions. Differing from most of the existing literature, our framework is \textit{user-aware}, i.e., it allows users to quit the simulation, either if the suggestions are not relevant or if they get bored, and eventually compute the diversity obtained over the final set \seenitems of picked interactions. Notably, in this way, we induce a strong interplay among \textit{relevance}, \textit{diversity}, and \textit{user behavior}, whose rationale is depicted in Figure~\ref{fig:toy_example}. Indeed, if the recommendation strategy focuses on utility only, i.e., it provides highly relevant but poorly diverse suggestions, then the user will not quit the simulation but the final diversity score will be low; vice-versa, if the recommendations are extremely diverse but low-quality, the user will immediately abandon the simulation process, hence resulting in a low final score as well. Thus, with our methodology, we ensure to account for the best trade-off between relevance and diversity.
\fi 

\smallskip
Motivated by the previous example, 
we propose a novel framework to model the behavior of the user
while exploring information via recommendations. 
Relevance is taken into account to model termination of exploration, 
but the overall quality is measured by a diversity measure.
We instantiate our model using two standard notions of diversity, 
one based on coverage and the other based on pair-wise distances~\cite{dum, mmr, dpp}.

Both diversity notions, coverage and pairwise distances, 
can be defined using an underlying space of user-to-item ratings or categories/topics. 
Other diversity notions can also be incorporated into our framework, 
e.g., pair-wise distances of item embeddings, obtained by representation learning, 
but we leave this for further study, as it is not our focus.

Finally, we propose a novel recommendation strategy 
that combines relevance and diversity by a copula function. 
We perform an extensive evaluation of the proposed framework and strategy using five benchmark datasets publicly available, and show that our strategy outperforms several state-of-the-art competitors.

% This given, in this work, we address the presented problem by ($i$) developing a novel simulation framework that relies on both accuracy and diversity, ($ii$) defining two measures to be applied to the final set of user interactions, and ($iii$) implementing two recommendation strategies that prove to be effective in this context.

Our contributions are summarized as follows:
\begin{itemize}
    \item We develop a user-aware framework that models information exploration via recommendations; 
    our framework takes into consideration the interplay among relevance, diversity, and user behavior.
    \item We instantiate our framework with two diversity measures, defined over user-to-item ratings or categories/topics.
    \item We propose a recommendation strategy that accounts for both diversity and accuracy when providing suggestions.
    \item We conduct an extensive analysis over multiple benchmark datasets and several competitors to show the effectiveness of our proposal in the suggested framework.
\end{itemize}

The rest of the paper is structured as follows. Section~\ref{sec:related} presents the related work in terms of user modeling and diversity in recommendations. Section~\ref{sec:problem} presents our problem definition and methodology. In Section~\ref{sec:our_strategies} we present our recommendation strategy. Experimental results are reported in Section~\ref{sec:experiments}, and finally Section~\ref{sec:conclusion} concludes the paper and provides pointers for future extensions. 

\begin{comment}
\section{Related work - Giuseppe}


% \aris{Writing tip: 
% Do not use citations as nouns.
% E.g., never say ``[8] did this'', instead say ``Coppolillo et al. [8] did this''.
% An easy way to do this is by using the command \texttt{{\textbackslash}citet} when the citation is used as a noun, 
% and \texttt{{\textbackslash}citep} when the citation is silent.}

\spara{User modeling in recommender systems.} 
The effects of user behavior in recommender systems, in terms of novelty and diversity, have gained a lot of attention in recent years. Analysis can be conducted by either running user studies, hence observing actual user choices~\citep{Lee2014ImpactOR, recsys_sales_diversity, sales_diversity_impact, Zhu2018TheIO}, or by means of simulation~\citep{simulating_impact, diversity_under_users_modeling, Yao2021MeasuringRS}. %Examining the decisions made by real users can lead to more reliable results, but it introduces the challenge of developing a functional recommendation system and conducting extensive user~studies. 
Analyzing the choices made by actual users can yield more dependable outcomes; however, it also requires creating an effective recommendation system and engaging users for conducting comprehensive studies. 
%which can be highly consuming, both in terms of time and resources. 

Conversely, simulating user choices offers a more straightforward approach, enabling the testing of multiple system configurations without incurring costs; nevertheless, it necessitates an accurate model of emph{user behavior}.
To address this challenge, several user-behavior models have been proposed in the literature. 
\citet{HAZRATI2022102766} model the probability that a user picks a recommended item 
as being proportional to the utility of the item.
%  scaled by a factor representing the uncertainty in its estimation and boosted by a multiplicative factor.
Similarly, \citet{siren} propose a simulation framework in which users decide to interact with a certain number of items per iteration, according to their given preferences. 
\citet{diversity_under_users_modeling} present three different user-behavior models, 
by imposing that users either blindly follow recommendations and choose the most popular items, 
or completely ignore suggestions and pick items randomly. 

The previously mentioned models have some inherent limitations. Firstly, they require users to select an item, meaning users cannot simply exit the application. Secondly, these models maintain a constant selection probability over time, failing to account for the gradual decline of interest due to irrelevant recommendations or the passage of time.

To address these limitations, we introduce a \textit{quitting probability} into our model. This allows users to interrupt their interaction with the recommender system. We hypothesize that the likelihood of quitting depends on both the utility of the recommended items and the user's \textit{patience}, which decreases as time passes.
Notably, with our framework, we leverage the intrinsic interplay among relevance, diversity, and user behavior, 
since successful recommendation strategies need to ensure that they provide recommendations that are both relevant and diverse.
%  the final score (i.e., the diversity obtained over the user items set) will be low either if the interactions are relevant but not diverse, or, vice-versa, if the suggested items are highly different but low-quality, thus inducing users to quit the simulation (and so the final items' set to be small).

\aris{The next paragraphs conflate diversity in information retrieval and diversity in recommender systems, 
i.e., MMR was designed for IR.
Are these two the same?
I think that we should make a distinction.}
\erica{I think I did not get what you mean. IR and recommender systems are quite related concepts. What should be the distinction in your opinion?}

\aris{Why we say that \citet{first_diversification} is the first diversity approach, 
if MMR \citep{mmr} is much older?
Is it IR vs.\ RS?}
\erica{Yes. MMR was born to diversify the keywords of a document in order to avoid redundancy. \citet{first_diversification} were the first to embrace the concept of diversity in recommender systems (I found this information in another paper. If you think it is misleading I can rephrase it).}


\spara{Diversity in recommender systems.}  
The challenge of striking a balance between diversity and utility (relevance) has been extensively explored in the broader domain of information retrieval. Various re-ranking strategies have been devised to address this issue. One such approach is the "maximal marginal relevance" (MMR) method, as described by \citet{mmr}. MMR employs a weighted linear combination of scores that evaluate both utility and diversity, offering a systematic way to address this critical aspect of recommendation systems.

In the specific context of recommender systems, \citet{first_diversification} introduced one of the earliest methods for enhancing diversity. They achieved this by employing a greedy selection approach, where they picked items that minimized the similarity within a recommended list.

Addressing the challenge of balancing accuracy and diversity, \citet{accuracy-diversity_dilemma} proposed a solution based on random walks. They tackled what is commonly referred to as the "accuracy-diversity dilemma," which involves finding an optimal trade-off between these two measures.
This concept is also recognized as "calibration," as mentioned by \citet{calibration}. Calibration pertains to the algorithm's ability to provide recommendations that avoid neglecting the user's secondary areas of interest and ensure they are adequately represented.
%In the literature of information retrieval, several re-ranking strategies have been proposed for achieving a good balance between diversity and utility: the \emph{maximal marginal relevance} (MMR) method~\citep{mmr} adopts a weighted linear combination of utility and diversity scores; 
\citet{dum} propose to greedily select items by maximizing the utility via a submodular function. \citet{dpmf} suggest to optimize the diversity loss of items using probabilistic matrix factorization. \citet{dpp} propose a determinantal point process (DPP) to re-rank the recommended items so as to maximize the determinant on the items' similarity~matrix. 

In their research, \citet{diverse_content} investigate the impact of diversity on music ranking for consumption. They introduce two innovative models: a feed-forward neural ranker and a reinforcement learning-based ranker. The former model incorporates a dynamic user embedding by considering the user's previous sessions. In contrast, the latter model defines rewards based on the user's assessment of track relevance.

Reinforcement learning also plays a role in the study conducted by \citet{multi-armed}, where diversity is introduced through the use of multi-armed bandits during the elicitation phase. Additionally, in the work by \citet{linear_bandits}, they propose an online learning framework to optimize diversified retrieval by carefully balancing the exploration and exploitation of users' preferences and interests.

However, it's worth noting that these reinforcement learning-based approaches typically require a lengthy training phase, which can often be prone to stability issues. This is in contrast to our approach, which may offer a more efficient and stable solution.
% \citet{diverse_content} investigate how ranking affects diversity in music consumption, thus proposing two novel models, 
% namely, a feed-forward neural ranker and a reinforcement learning-based ranker. The former incorporates the user’s
% previous sessions to produce a dynamic user embedding. By contrast, the latter defines the reward based on whether the user found the track to be relevant.
% Reinforcement learning was also been adopted in the work by \citet{multi-armed}, 
% where diversity is induced by adopting multi-armed bandits in the elicitation phase.
% \citet{linear_bandits} propose an online learning setting for optimizing diversified retrieval in terms of covered topics, by balancing exploration and exploitation of users' tastes.

\aris{For all the works above that use RL \citep{diverse_content, multi-armed, linear_bandits}, 
how they differ from our approach? More details are needed.}
\erica{RL techniques are based on a (generally really long) training phase based on a reward function, thus being a completely different approach. Do you want me to be more technical in explaining how the reward function is modeled in the cited papers?}

%\aris{Do not use acronyms without defining them, e.g., VAE. Also no need to use acronyms at all a term that is used only one time.}

Several other \emph{neural-network models} have been applied to address the diversity problem. 
\citet{diversification_vae_based} adopt a \emph{variational auto\-encoder} to induce targeted (i.e., topical) diversity. 
\citet{enhancing_adaptivity} propose a \emph{bilateral branch network} to achieve a good trade-off between relevance and diversity, defined at either domain or user level. 
\citet{dgcn} present a \emph{graph neural network} for diversified recommendations, 
where node neighbors are selected based on inverse category frequency, 
together with negative sampling for inducing diverse items in the embedding space.

\aris{How do these NN methods compare with our method?
Do they compete with our method?}
\erica{They do, since they optimize diversity (either in terms of distance or coverage) in their loss function. Indeed, we use the last cited one as a competitor.}

% We argue that the reported approaches are either highly demanding in terms of time and/or computational resources, or rely on some heuristics not theoretically justified.

\giuseppe{I would not mention the copula here. The main technical contribution does not rely on the copula, but on the assumption that relevance only plays a main role in user behavior, thus we can optimize diversity while staying in the context of high relevance. }
\textcolor{red}{We propose a novel recommendation strategy, namely \ouralgo, that accounts for both relevance and diversity, either at item- or group-level. Notably, our algorithm does not need any sort of training or hyper-tuning (\erica{we have to say it somewhere}) and is not time-consuming \erica{times plot is in the Appendix}. It indeed ensures to provide both highly-relevant and diverse suggestions, by exploiting the properties of the Clayton copula function~\cite{clayton_copula}. To the best of our knowledge, ours is the first attempt to adopt copulas in this context.}

\giuseppe{Alternate formulation: \\
In contrast to the approaches mentioned earlier, the recommendation strategy we introduce, referred to as \ouralgo, does not necessitate any form of training or hyperparameter tuning. Instead, it operates on the premise that user engagement is primarily governed by relevance. Consequently, we aim to strike an effective balance with diversity by optimizing it independently within the context of high relevance, computed separately. We outline the formalization of our approach in the following sections.}
\end{comment}

